Game Semantics: Easy as Pi

Game semantics has proven to be a robust method to give compositional semantics for a variety of higher-order programming languages. However, due to the complexity of most game models, game semantics has remained unapproachable for non-experts. In this paper, we aim at making game semantics more accessible by viewing it as a syntactic translation into a session typed pi-calculus, referred to as metalanguage, followed by a semantics interpretation of the metalanguage into a particular game model. The syntactic translation can be defined for a wide range of programming languages without knowledge of the particular game model used. Simple reasoning on the model (soundness, and adequacy) can be done at the level of the metalanguage, escaping tedious technical proofs usually found in game semantics. We call this methodology programming game semantics. We design a metalanguage (PiDiLL) inspired from Differential Linear Logic (DiLL), which is concise but expressive enough to support features required by concurrent game semantics. We then demonstrate our methodology by yielding the first causal, non-angelic and interactive game model of CML, a higher-order call-by-value language with shared memory concurrency. We translate CML into PiDiLL and show that the translation is adequate. We give a causal and non-angelic game semantics model using event structures, which supports a simple semantics interpretation of PiDiLL. Combining both of these results, we obtain the first interactive model of a concurrent language of this expressivity which is adequate with respect to the standard weak bisimulation, and fully abstract for the contextual equivalence on second-order terms. We have implemented a prototype which can explore the generated causal object from a subset of OCaml.

==> det.tex <==
%! TEX root = main.tex
"Strategies" presented in \S~\ref{sec:lindet} are linear: each move of
the game can be played at most once in an execution. As moves
correspond to function calls, we are restricted to interpreting linear languages.

In this section, we extend our framework to handle nonlinear
computations, following the methodology of \citet{lics15, cg2}. In
\S~\ref{sec:nonlinexp}, we present the challenge of extending the
previous setting to deal with non-linearity. In \S~\ref{sec:ess}, we
recall "event structures with symmetry", the technical tool used to
solve this issue. In \S~\ref{sec:detstrat}, we present how to build a
category out of these ideas. In \S~\ref{sec:ccll}, we present $\PILL$,
an extension of $\PIMALL$ with the exponentials of Linear Logic to
define nonlinear strategies. In \S~\ref{sec:cbn} and \S~\ref{sec:cbv},
we look at encodings of higher-order languages into $\DetStrat$
following game semantics methodology, both in call-by-name and
call-by-value.

\subsection{Non-linearity in Game Semantics}\label{sec:nonlinexp}
A standard procedure to interpret nonlinear computations inside a
linear model is given by Linear Logic \cite{girard1987linear}. The
main insight is that for each type $A$, there should be two types
$\oc A$ and $\wn A$ allowing repeated invocations of $A$. In this
setting, an object of type $\oc A$ should be seen as producing
infinitely many $A$'s, while an object of type $\wn A$ as producing
finitely (possibly zero) $A$'s. This is well-behaved when it comes to
interaction since a $\oc (A^\perp)$ is a morally a ``server'', able to
consume infinitely many $A$'s, while $\wn A$ is a client, issuing
several requests of type~$A$.

\citet{Seely89} defines the algebraic structure required on these new
objects. By duality, it is enough to describe the structure for one of
those two connectives. First $\wn A$ should be a monad conform to the
intuition that $\wn A$ is a bundle of many $A$'s; and moreover it must
turn any object into a commutative comonoid, i.e. for every~$A$, it
must come equipped with a map
$\wn A \parallel \wn A \rightarrow \wn A$ explaining how to join bags
together (and a unit $1 \rightarrow \wn A$, the empty bag).

Before building such structure in games and strategies,
let us look at the category of event structures first (indeed, most of
the structure can be "lifted@lifting of maps" to strategies).
%
In event structures, a candidate for ``infinite many $E$'s'', is the
following construction. Given an event structure $E$, we define
$\intro*{\sharpG E}$ as $ \parallel _{i \in \mathbb{N} } E$. In particular,
its events are pairs $(i, e)$ of a move $e \in E$ and an integer
$i \in \mathbb{N} $, referred to as a ""copy index"".
%
There are natural candidates for a monad structure on $\sharpG {(-)}$:
$$
   \eta _E: (a \in E) \mapsto (0, a) \in \sharpG E \qquad \qquad \mu _E: \big((i, (j, a)) \in \sharpG {\sharpG E}\big)  \mapsto \big((\EncodingPairs {i, j}, a) \in \sharpG E\big) \\
$$
where
$\intro*{\EncodingPairs {\cdot, \cdot}} : \mathbb{N} ^2 \simeq
\mathbb{N} $ is any bijection. To satisfy the monadic laws, we must
have $\EncodingPairs {0, i} = \EncodingPairs{i, 0} = i$ for all
$i \in \mathbb{N} $, which is incompatible with
$\EncodingPairs{\cdot, \cdot}$ being a bijection. There is in fact no
hope of realising these laws ``on the nose'', i.e. up to function
equality.  Instead, the equation holds \emph{up to "copy
  indices"}. This is reasonable: the precise identity of copy indices
should not affect the semantics since they are an artefact of the
model. To formalise the notion of equality ``up to copy indices'', we
equip $\sharpG E$ with an "isomorphism family", turning it into an
"event structure with symmetry".


\subsection{Event Structures with Symmetry} \label{sec:ess} 
The main idea of event
structures with symmetry introduced by \citet{winskel2007event}
is not to look at events
individually but at configurations instead.

\begin{definition}
  An ""isomorphism family"" on an event structure $E$ is a family
  $\tilde E$ of order\-/isomorphisms $ \varphi : x  \cong  y$ with $x, y  \in   \config (E)$ such
  that
  \begin{enumerate}
  \item $\tilde E$ contains all identities, and is stable under inverse and composition
  \item If $x \subseteq x'$ and $ \varphi  : x'  \cong  y'  \in  \tilde E$, then $ \varphi \vert_x : x  \cong   \varphi \, x \in \tilde E$
  \item If $x \subseteq x'$ and $ \varphi  : x  \cong  y \in \tilde E$, then there
    exists a (non-necessarily unique) $y' \in \config(E)$ such that $ \varphi $
    extends to $ \varphi ' : x'  \cong  y' \in \tilde E$.
  \end{enumerate}
%
  An ""event structure with symmetry"" is a pair $(E, \tilde E)$ of an
  event structure $E$ and an "isomorphism family" $\tilde E$ on $E$.
We write $\mathcal E, \mathcal F, ...$ for "event structures with
symmetry".  
\end{definition}
Most constructions on event structures (such as "parallel
composition", "sum" and "lifting") can be extended seamlessly to "event
structures with symmetry" \cite{winskel2007event}. Given an event
structure with symmetry $\E$, define an isomorphism family
$\sharpG \tilde E$ on $\sharpG E$ containing all the $ \theta : x \cong y$ for which
there exists $ \pi : \mathbb{N} \rightarrow \mathbb{N} $ such that
$$(1)\, \text{for $(i, e)  \in  x$, $ \theta \, (i, e)$ is of the form $( \pi \, i, e')$}
\qquad \text{and}\qquad
(2)\, \{ (e, e') \mid \theta (i, e) = ( \pi \, i, e') \} \in \tilde E.$$
We
define the "event structure with symmetry" $\sharpG \E$ as
$(\sharpG E, \sharpG \tilde E)$.

A ""map of event structures with symmetry"" $f : \mathcal E  \rightharpoonup
\mathcal F$ is a "map" $f : E  \rightharpoonup  F$ such that for all $ \theta
\in \tilde E$, $f\, \theta \eqdef \{ (f\, e, f\, e') \mid (e, e') \in \theta \}$
is in $\tilde E$. Two such "maps@mapess" $f, g : \E \rightarrow \F$ are said to
be ""similar"" if for all $x \in \config (E)$, $\{ (f\, s, g\, s) \mid s \in x\} \in
\tilde E$, which we write $f \similarMaps g$. Event structures with symmetry and
total maps form a category $\intro*{\ESS}$.
%
This equivalence relation is enough to formalise this idea of equality
up to copy indices.
\begin{lemma}
  $\sharpG {(-)} : \ESS \rightarrow \ESS$ is a monad up to
  $\similarMaps$.
\end{lemma}

%In the next section, we show how to extend strategies to work with
%symmetry.
\subsection{The Category $\DetStrat$}\label{sec:detstrat}
\subsubsection*{Games with Symmetry} To be able to identify strategies
up to copy indices, we need more structure than a simple symmetry on
$A$, but the structure of a "thin concurrent game" \cite{cg2}.

\begin{definition}
  A ""thin concurrent game"" (tcg) is a tuple
  $\A = (A, \tilde A, \tilde A_+, \tilde A_-)$ where $A$ is a game,
  and $\tilde A, \tilde A_+, \tilde A_-$ are isomorphism families on
  $A$ subject to axioms listed in \cite{cg2}; in particular
  $\tilde A_-$ and $\tilde A_+$ are sub-isomorphism families of $\tilde A$.
\end{definition}
The intuition is that $\tilde A_-$ (resp. $\tilde A_+$) contain only
isomorphisms that affect negative (resp. positive) events. This idea of
polarised decomposition of the symmetry was first introduced by
\citet{mellies2003asynchronous} in a simpler setting. Games operations (parallel composition, dual) extend to tcgs.
\subsubsection*{Uniform Strategies} Symmetry on games induces
naturally an equivalence relation on strategies, relaxing
"isomorphism" by asking that the triangle commutes up to symmetry on
the game. This equivalence, however, is not a congruence since nothing
prevents a strategy to observe copy indices from Opponent. To recover
a well-behaved compositional setting, we need to ensure that the
strategy we consider behaves uniformly with respect to copy indices
from Opponent. It turns out that we need to add extra structures on
strategies, under the form of an isomorphism family.

\begin{definition}
  Consider a "tcg" $\A$.  A ""uniformity witness"" for
  $ \sigma  : S  \rightarrow  A$ is an isomorphism family $\tilde S$ on $S$ such that:
  \begin{enumerate}
  \item $ \sigma $ becomes a "map of event structures with symmetry"
    $(S, \tilde S) \rightarrow  (A, \tilde A)$;
  \item if $ \theta  : x  \cong  y \in \tilde S$ and $ \sigma \,  \theta $ extends to
    $ \varphi  : x'  \cong  y' \in \tilde A$ with $x \subseteq^- x'$, then $ \theta $ extends
    to a $ \theta '$ such that $ \sigma \,  \theta ' =  \varphi $;
  \item if $ \theta  : x  \cong  y \in \tilde S$ is the identity on negative
    elements of $x$, then $ \theta $ is the identity on $x$.
  \end{enumerate}
  A ""$\sim$-strategy"" on $\A$ is a "strategy" $ \sigma $ on $A$ along with a
  "uniformity witness" for $ \sigma $.
\end{definition}

\noindent
We can lift the equivalence relation $\similarMaps$ on "maps@mapess" to a weak
isomorphism on strategies: two "$\sim$-strategies" $ \sigma  : S  \rightarrow
A$ and $ \tau  : T  \rightarrow  A$ are ""weakly isomorphic"" (written $ \sigma
\weakIso  \tau $) when there exists an isomorphism of "event structures with
symmetry" $ \varphi  : \mathcal S  \cong  \mathcal T$  such that $ \tau  \circ
\varphi  \similarMaps  \sigma $.

\begin{theorem}[\cite{cg2}]
  Uniformity witnesses compose and "weak isomorphism" is a congruence
  on $\sim$-strategies. As result, "tcgs" and "$\sim$-strategies" up
  to "weak isomorphism" form a compact-closed category
  $\intro*{\DetStrat}$.
\end{theorem}

\subsubsection*{The Lifting Monad} Unfortunately, if $\A$ is a "tcg",
$\sharpG \A$ is not a "tcg" is general. However, if $\A$ is
"polarised" then $\sharpG \A$ is also "tcg" \cite{cg2}. To work around
this issue, we lift games before taking $\sharpG {(-)}$ which leads to
the two natural exponentials of Linear Logic: $\ocG \A$ (resp.
$\wnG \A$) when lifted with a negative (resp. positive) move.

Formally, liftings of games are defined as follows. Given a "tcg"
$\A$, we define $\intro*{\LiftNeg{\mathcal A}}$ to be the "tcg"
$\mathbf{box}^- \cdot \A$. This operation on "tcgs" extends to a
functor $\LiftNeg - : \DetStrat \rightarrow \DetStrat$: given
$ \sigma : \A \profto \B$, $\LiftNeg { \sigma }$ starts by
acknowledging the negative \texttt{box} on the right, before playing
\texttt{box} on the left, and continuing as $ \sigma $. As a result,
$\LiftNeg { \sigma }$ is a "negative strategy". Writing $\DetStrat^-$
for the subcategory of $\DetStrat$ whose games are "negative@negative
game" with "negative strategies" on it, we have:

\begin{restatable}{lemma}{adjunt}\label{lemma:adjunt}
  The functor $\LiftNeg {(-)}$ is the right adjoint to the inclusion
  $\DetStrat^-  \rightarrow  \DetStrat$.
  %
  In particular, $\LiftNeg$ transports comonads on $\DetStrat^-$ to
  comonads on $\DetStrat$.
\end{restatable}
By duality, we define similarly $\intro*{\LiftPlus \A}$ which has a
dual adjunction result.
\subsubsection*{Exponentials on $\DetStrat$} On $\DetStrat^-$,
$\sharpG{(-)}$ has the desired structure:
\begin{lemma}[\cite{cg2}]
  $\sharpG{(-)} : \DetStrat^- \rightarrow \DetStrat^-$ is an
  ""exponential comonad"", i.e.\ in this affine setting, a comonad
  equipped with a natural transformation, the ""contraction"",
  $\contraction \A : \sharpG \A \profto \sharpG \A \parallel \sharpG \A$ which turns
  $\sharpG \A$ into a comonoid.
\end{lemma}

\noindent
The exponential comonad $\sharpG{(-)}$ induces, through the lifting
adjunction, an exponential comonad $\ocG{(-)}$:
$\intro*{\ocG{A}} = \sharpG {\LiftNeg A}$.  By duality, we get the
exponential monad $\intro*{\wnG {\A}} \eqdef \sharpG {\LiftPlus
  \A}$. The unit of the monad $\wnG{(-)}$ gives the ""dereliction""
strategy ${\dereliction \A} : \A \profto \wnG \A$, forwarding $\A$
onto the zeroth copy of $\A$ in $\ocG \A$; and the multiplication of
the comonad $\ocG{(-)}$ gives the ""digging"" strategy
${\digging \A} : \oc \A \profto \oc \oc \A$, forwarding
$( \langle i, j \rangle , a)$ onto $(i, (j, a))$.


\subsection{A Metalanguage for $\DetStrat$: $\PILL$}\label{sec:ccll} 
To build a calculus for $\DetStrat$, we extend the calculus of
\S~\ref{sec:mall} with the exponentials of Linear Logic:
$$
T \Coloneqq ... \mid \oc T \mid \wn T
\quad \quad  
P \Coloneqq \cdots \mid \Prom a x.\, P \mid \Der a x.\, P \mid \Contr a {x} {y}.\, P
$$
The type $\oc T$ represents a \emph{server} waiting for clients
following protocol $T$ and the type $\wn T$ is for a \emph{client}
connecting to a server that follows protocol~$T$. The process
$\Prom a x.\, P$ creates a \emph{server} listening on~$a$; spawning a
copy of $P$ for every request $x$ made; $\Der a x.\, P$ is a \emph{client}
which connects to server~$a$ and continues as~$P$ with channel~$x$
meant to perform the request. The process $\Contr a {x} {y}.\, P$ is a
\emph{duplication}: it duplicates the name~$a$ into two names~$x$
and~$y$ and executes~$P$: the two names will be connected to the same
server but can issue requests in parallel to the server. This
construction allows the non-affine use of channels of type $\wn
T$. Note that $\fc{\Contr a {x} {y}.\, P} = \fc{P}\setminus
\{x,y\}$. Typing judgements are extended with the corresponding rules
of Linear Logic:
$$\inferrule*[left=Server]
  {\Typing {P} {\wn  \Gamma , x: T}}
  {\Typing{\Prom a x.\, P} {\wn  \Gamma , a: \oc T}}
  \quad
  \inferrule*[left=Client]
  {\Typing{P}{ \Gamma , x: T}}
  {\Typing{\Der a x.\, P} { \Gamma , a: \wn T}}
  \quad
  \inferrule*[left=Dup]
  {\Typing{P}{ \Gamma , x: \wn T, y: \wn T}}
  {\Typing{\Contr a x y.\, P} { \Gamma , a: \wn T}}
$$
Rule {\sc{Server}} ensures that all the free names of an exponential input are
client names (denoted by $?\Gamma$); rule {\sc{Client}} types a request (once)
to a server; and Rule {\sc{Dup}} types a duplicator where the type of $x,y$ is
the same as $a$. The forwarder can naturally be extended:
$$\Forwarder a b {\oc T} = \Prom a x.\, \Der b y.\, \Forwarder x y T.$$

\subsubsection*{Infinitary terms} Types now denote infinite games, and
as a result the model contains infinite strategies. The promotion
construction allows to define some infinite strategies, but it is not
enough. To allow arbitrary infinite behaviours, we consider
\emph{infinite terms} with \emph{infinite typing
  derivations}. Formally, we consider the free $ \omega $-CPO over the
set of typing derivations, ordered by prefix. This will be useful to
interpret the fixpoint operator of $\PCF$ and the memory allocation of
$\PCFM$.


\subsubsection*{Interpretation of the Calculus} Types are interpreted
by the corresponding operations in $\DetStrat$ homomorphically:
$\llbracket \oc T \rrbracket = \ocG  \llbracket T \rrbracket$ 
and $\llbracket \wn T \rrbracket = \wnG \llbracket T \rrbracket$.
The interpretation of the new process constructions follows the
standard categorical semantics of Linear Logic:
$$
\small
\!\!\!\!\begin{array}{c}
\left\llbracket\vcenter{
  \infer
  {\Typing{\Prom a x.\, P} {\wn  \Gamma , a: \oc T}}
  {\Typing {P} {\wn  \Gamma , x: T}}}
\right\rrbracket =
(\ocG \llbracket P \rrbracket : \ocG \ocG  \llbracket  \Gamma  \rrbracket^\perp \profto \ocG  \llbracket T \rrbracket)  \odot  \digging {\llbracket  \Gamma  \rrbracket^\perp}
\ 
  \left\llbracket\vcenter{
  \infer
  {\Typing{\Der a x.\, P} { \Gamma , a: \wn T}}
  {\Typing{P}{ \Gamma , x: T}}}
\right\rrbracket =
\dereliction {\llbracket T \rrbracket} \odot  ( \llbracket P \rrbracket :  \llbracket  \Gamma  \rrbracket^\perp \profto  \llbracket T \rrbracket)
\\[1mm]
\left\llbracket\vcenter{
      \infer
      {\Typing{\Contr a x y.\, P} { \Gamma , a: \wn T}}
      {\Typing{P}{ \Gamma , x: \wn T, y: \wn T}}
    }
    \right\rrbracket
    =
    \contraction { \llbracket T \rrbracket}  \odot  ( \llbracket P
    \rrbracket :  \llbracket  \Gamma  \rrbracket^\perp \profto \wnG
    \llbracket T \rrbracket  \parallel  \wnG  \llbracket T \rrbracket)
\end{array}
$$
The interpretation of infinitary terms follows from this result:
\begin{lemma}[\cite{lics15}]
  For any "tcg" $A$, "$\sim$-strategies" over $A$ have a natural order
  which turns $\DetStrat(A)$ into an $ \omega $-CPO. 
\end{lemma}
\noindent
The interpretation of finite terms of $\PIMALL$ into $\DetStrat$ is
monotonic for this order, and as a result, can be uniquely extended by
continuity to infinite terms.

\subsubsection*{Equational Theory} We extend "open processes@open process" as follows:
$$\OpenProc \Coloneqq \cdots \mid \Prom a x.\, \OpenProc \mid \Contr a {a_1} {a_2}.\, \OpenProc \mid \Der a x.\, \OpenProc$$
The action $\Contr a {a_1}{a_2}.\, X$ is a naming action;
$\Prom a x.\, X$ is a negative one; and $\Der a x.\, X$ is positive.
%
We use the following macro to manage context duplication, where
both processes have access to the same channels
%
\[
  \share \Gamma P Q \eqdef \Contr{\vec x}{\vec a}{\vec b}.\;
  \left(
    P\subst{\vec x}{\vec a}
    \parallel
    Q\subst{\vec x}{\vec b}
  \right)
\quad\mbox{such that}\quad 
  \vcenter{\prftree
  {\Typing P {\wn \Gamma, \Delta_1}}
  {\Typing Q {\wn \Gamma, \Delta_2}}
  {\Typing {\share \Gamma P Q} {\wn \Gamma, \Delta_1, \Delta_2}}}
\]
We also use $P[a^?]$ for $\Der a x.\, P[x]$ to limit the noise added
by derelictions.

In {\bf Communication}, the first rule is defined as a usual reduction
for the $\pi$I-calculus \cite{DBLP:journals/tcs/Sangiorgi96a}; the
second rule creates two fresh servers which are accessed by $Q$.  In
{\bf Contractions}, the rules are there to reflect the fact that
contraction induces a comonoid structure.

Note that the communication rule for $\oc/\wn$ makes the server disappear,
unlike the usual replication rules in the $ \pi $-calculus. The typing rules
ensure that there are no occurrences of~$a$ in~$Q$: the server will never be
contacted again and hence can safely be shut down. The only way to contact a
server twice is via the use of the contraction rule, which will duplicate the
server accordingly.

\begin{figure}[t]
\small
{\bf Communication}\\[1mm]
\begin{tabular}{l}
    %% Communication
    % 1.  \Prom/dereliction
$ \cut a b {\oc T} {(\Prom a x.\, P \parallel \Der b y.\, Q)}
      \similarProcesses
      \cut x y {T} {(P \parallel Q)}$\\[1mm]
    % 2.  \Prom/contraction
$\cut a b {\oc T} {(\Prom a x.\, P \parallel \Contr b {b_1} {b_2}.\, Q)}
      \similarProcesses
      \cut {a_1} {b_1} {\oc T} {\cut {a_2} {b_2} {\oc T}
{((\share {\Delta} 
{\Prom {a_1} x.\, P} {\Prom {a_2} x.\,  P}) \parallel Q}})$\\
\hspace{7cm}{\footnotesize (if $\fc P \setminus \{x\} =  \Delta$, 
                   $(\fc{P}\cup \fc{Q})\cap \{a_1,a_2\}=\emptyset$)}\\[1mm]
\end{tabular}
{\bf Contractions}\\[1mm]
\begin{tabular}{l}
$\Contr a {a_1} {a_2}. \, P \similarProcesses \Contr a {a_2} {a_1}.\,
P$
\quad \quad 
$\Contr a {b} {a'}. \, \Contr {a'} {c} {d}.\, P \similarProcesses
\Contr a {a'} {d}.\, \Contr {a'} {b} {c}.\, P$\\[1mm]
$\Contr a {b} {c}. P \similarProcesses P [a/b]$ 
{\footnotesize (if $c \not\in \fc P$)}
\end{tabular}
  \caption{Equational Theory for $\PILL$}
  \label{fig:eqtheoryLL}
\end{figure}

\begin{restatable}[Soundness]{lemma}{detsoundness}
If $P \similarProcesses Q$, then $ \llbracket P \rrbracket  \cong   \llbracket Q \rrbracket$.
\end{restatable}



\subsection{Interpretation of Call-by-Name PCF in $\DetStrat$}\label{sec:cbn}
We show how to translate a non-linear language, PCF, into 
$\PILL$. 
%
The grammar of types and terms extends that of the affine
$ \lambda $-calculus.
$$\begin{aligned}
  \tau \Coloneqq  \cdots \mid  \mathbb{N} 
  \qquad
  M \Coloneqq \cdots \mid \mathtt{n} \in \mathbb{N} \mid \mathbf{Y} \mid 
  \mathtt{iszero}(M) \mid \mathsf{succ}(M)
\end{aligned}$$ The typing rules of PCF are standard. We write
$ \rightarrow _{\PCF}$ for the standard call-by-name reduction on
terms of PCF. Due to the non-linearity, we change the interpretation
of the arrow to use an exponential on the argument:
$$\transl { \tau _1 \to  \tau _2} = \oc \transl{ \tau _1} \linto \transl{ \tau _2} \qquad \transl{ \mathbb{N} } = \start^- \cdot \oplus_{n  \in   \mathbb{N} } \EmptyType \qquad \transl{ \mathbb{B} } = \start^- \cdot \oplus_{b  \in  \{\ttrue, \ffalse\}} \EmptyType.$$

The translation on terms is then updated to take non-linearity into
account, following the usual encoding of call-by-name computation into Linear Logic. It is described in Figure~\ref{fig:translation-cbn-pcf}.
%
\begin{figure}
\textbf{Translation of Terms}
{\small
\begin{align*}
  \transl { \Gamma , x:  \tau   \vdash  x: \tau}_i ^o
  &\quad \eqdef \quad 
    \Der x u.\, \Output x i.\, {\Forwarder u o {\tau / i}}
  \\
  \transl{ \Gamma   \vdash  \abs x M: \tau_1 \to \tau_2}^o_i
&\quad \eqdef \quad 
    \Naming o {x, o}. \transl M^o_i
  \\
  \transl {\app{M}{N}: \tau_2}^o_i
&\quad \eqdef \quad 
    \shareInteract x y {\transl  \Gamma }
    {\Split o {x, o} {\transl M^o_i}}
    {\Prom x r.\, \transl N^r}
   \\
   \transl{\ifte M N {N'} : \tau}^o_i
&\quad \eqdef \quad 
      \shareInteract x {y} {\transl \Gamma}
        {\transl M^x_\Start}
        {\InputII {y} {} {\ttrue: \transl N^o_i; \ffalse: {\transl {N'}^o_i}}}
   \\
   \transl{\mathbf{Y}: (\tau \to \tau) \to \tau}^o_i
&\quad \eqdef \quad 
                                                      \Naming o {f, u}.\, \mathsf{fix}^{f, u}_i
  \\
  \transl{\mathsf{iszero} :  \mathbb{N}   \rightarrow  \mathbb B}^o_\Start
&\quad \eqdef \quad 
    \Naming o {a, o}.\, \Output a \Start.\, 
                                               a \with\left\{
                                               \begin{aligned}
                                                 0:\, &\Output o \ttrue \\
                                                 n+1:\, &\Output o \ffalse \\
                                               \end{aligned}
  \right. \\
  \transl{\mathsf{succ} :  \mathbb{N}   \rightarrow  \mathbb N}^o
&\quad \eqdef \quad 
  \Naming o {a, o}.\, \Output a \Start.\, 
                                                                    \InputII a {n \in  \mathbb{N} } {n: \Output o {n+1}}
                                                                    \\[-1.5em]
%
\end{align*}
}

\textbf{Macros}

  {\footnotesize
  \[
  \begin{array}{rlll}
    \text{Name} & \text{Definition} & \text{Type}
    \\[1mm]
  \shareInteract a b \Gamma P Q
    &
  \cut a b \_ {(\share \Gamma P Q)}
    &
  {\wn \Gamma, \Delta_1, \Delta_2}
    \qquad \text{given}\ \ 
  {\Typing P {\wn \Gamma, \Delta_1, a: T}} \quad
  {\Typing Q {\wn \Gamma, \Delta_2}, b: T^\perp}
%
  \\[2mm]
    \mathsf{fix}^{u, f}_i
&
                            \begin{aligned}
                              &\Contr f {f_1} {f_2}.\, \Output {f_1^?} i.\, \Naming {f_1} {a, u'}.\\
                              &\quad (\Forwarder u {u'} {} \parallel \Prom a x.\, \InputII x {} {j.\, \mathsf{fix}^{x, f_2}_j})
                            \end{aligned}
& f: \wn (\transl { \sigma   \rightarrow   \sigma }^\perp), u:  \sigma /i                  
\end{array}
\]}

  \caption{Translation from call-by-name PCF to $\PILL$} 
  \label{fig:translation-cbn-pcf}
\end{figure}
%
This translation is similar to the one for the affine $\lambda$-calculus: apart
from adding a promotion in the definition of application, and a dereliction
for the variable case, we simply replaced instances of $\Interact x {\bar
x}{}{}$ with its non-linear counterpart.

\subsubsection*{Correctness} As before, we have the substitution lemma:
\begin{lemma}
  $\transl{M_1\subst{x}{M_2}}^o \similarProcesses \shareInteract x y \Gamma
  {\transl{M_1}^o}{\Prom y r.\,{\transl{M_2}^{r}}}$.
\end{lemma}

\begin{restatable}[Soundness and adequacy]{proposition}{PCFad}
  Given two terms $ \Gamma \vdash M, N : \tau$, if $M  \rightarrow _{\PCF} N$ then
  $\transl M^o \similarProcesses \transl N^o$. Moreover if
  $\transl M^o \similarProcesses \transl n^o$ for $ \vdash  M :  \mathbb{N} $, then
  $M  \rightarrow _{\PCF} n$.
\end{restatable}
\begin{proof}
  The proof of soundness is essentially the same as the affine case,
  using the fact that programs are interpreted by negative
  strategies. Adequacy is first proved on finite terms (terms without
  $Y$ but with immediate divergence), and then lifted to the infinite
  terms by continuity, following standard methods. The proof is in Appendix~\ref{sec:det-call-by-name-proof}
\end{proof}

Our methodology inherits the flexibility of game semantics. For
instance, for $\PCF$, we know that implementing \texttt{if}
concurrently, by evaluating the condition and the branches in parallel
leads also to a sound and adequate model, due to the absence of
state. We can describe such an interpretation here by simply changing
the interpretation of conditionals as follows:
$$\transl {\ifte M {N_1} {N_2}}^o_i =
(\nu u\, v; x_1\, y_1; x_2\, y_2)\left(
\begin{aligned}
  &\transl M^u_\Start \parallel_{\transl  \Gamma}  \transl {N_1}^{x_1}_i \parallel_{\transl  \Gamma } \transl {N_2}^{x_2}_i \\
  \parallel\, & \InputII v {} {\ttrue: \Forwarder {y_1} o {}; \ffalse: \Forwarder {y_2} o {}}
\end{aligned}
\right)
$$
The return value of $M$ is only used to know what value to return on
$o$: that of $N_1$ or that of $N_2$.
\subsection{Interpretation of Call-by-Value Languages in $\DetStrat$}\label{sec:cbv}
As an aside, to show that different encoding of types can lead to
different calling conventions, we show how to interpret a
call-by-value simply-typed $ \lambda $-calculus.
For simplicity and space reason, we
consider here PCF where the fixpoint combinator has been replaced by a
formal divergence $\bot : A$.
The fixpoint combinator in call-by-value is more
involved than in call-by-name and this simplification is
sufficient for demonstrating our framework. 
We use a standard call-by-value reduction whose main rules are:
$$\small \vcenter{\infer{( \lambda x.\, M)\, V  \rightarrow _v M \subst x V}{\text{$V$ is a value}}}
\qquad
\vcenter{\infer{\ifte b {M_{\ttrue}} {M_{\ffalse}}  \rightarrow _v M_b}{b \in \{\ttrue, \ffalse\}}}
\qquad
\vcenter{\infer{E[M]  \rightarrow _v E[N]}{M  \rightarrow _v N}}
\qquad+\text{rules for \texttt{iszero} and \texttt{succ}}
$$
where values and evaluation contexts are defined as follows:
$$V ::= n \mid b \mid  \lambda x.\, M \qquad
E ::= [] \mid E\, V \mid M\, E \mid \ifte E M N
\mid \mathtt{iszero}(E) \mid \mathtt{succ}(E).$$
The main difference between the game semantics interpretation of
call-by-name and call-by-value computations is the polarity of
types. In call-by-name, types become "negative games" waiting for a
message from Context before starting to evaluate; while in
call-by-value, types become "positive games" which can directly
produce a result.

Types of this language are interpreted as follows:
\[
  \transl {\mathbb B} = \oplus_{b \in \{\ttrue, \ffalse\}} \EmptyType 
  \qquad
  \transl {\mathbb N} = \oplus_{n \in  \mathbb{N} } \EmptyType 
  \qquad
  \transl {\oplus_{i \in I} A_i \to B} = \Lam^+ \cdot \oc {\with_{i \in I} (A_i^\perp
  \parallel  B)}.
\]
%
The translation of arrow types is more involved than in
call-by-name. The first move is played when the term has evaluated to
a closure. This is used to distinguish $ \lambda x. \bot$ and $\bot$;
only the first term will play $\Lam^+$. We then allow Context to call
this closure as many times as it wants (via the exponential $\oc$). To call the closure,
Context has to provide an argument value ($\with_{i \in I}$), and then
Program can ask further questions about its argument (playing in $A_i$) or
provide information about the return value (playing in $B$). For
instance, the type of functions from integers to
Booleans is interpreted as the game
$\Lam^+ \cdot \oc (\with_{n \in \mathbb{N}} \cdot (\ttrue^+ \oplus
\ffalse^+))$.

Remark that for all type $ \tau $, we have
$\transl \tau = \oplus_{i \in i} T_i$. The set $I$ is the set of
\emph{value types} of $ \tau $, written $\ValueType \tau $. Given
$i \in \ValueType \tau $, we write $ \tau /i$ for the type $T_i$. This
notation extends to contexts: we write $\ValueType {\Gamma}$ for the
set of families $(k_x)_{x \in \dom\Gamma}$ where
$k_x \in \ValueType {\transl { \Gamma (x)}}$. Given such a family
$(k_x)$, we write $ \Gamma /(k_x)$ for the \emph{metalanguage context}
$(x:  \Gamma (x)/k_x)_{x \in \dom  \Gamma }$.

We need this machinery because in call-by-value, terms receive values
from the context before starting to execute. As a result, the
translation works as follows: From a term $ \Gamma \vdash M : \tau $,
we build by induction a family of processes
$\Typing {\transl { \Gamma \vdash M : \tau }^o_{\vec k}} { (\Gamma
  /\vec k)^\perp, o: \transl \tau }$ indexed over value types of $ \Gamma
$. The translation is described in Figure
\ref{fig:translation-cbv-pcf}.

We can put these processes together using a specific tensor
product defined as follows:
$(\oplus_{i \in I}A_i) \otimes (\oplus_{j \in J}B_j) = \oplus_{i,j \in
  I \times J} (A_k \parallel B_l)$. For instance,
$\mathbb B \otimes \mathbb B$ is really a pair of booleans. We write
$\ctxTensor{\Gamma}$ for the tensor product of the interpretations of
the types in $\Gamma$: we have
$\ValueType{\otimes  \Gamma } = \ValueType  \Gamma $. The final translation is then
defined as follows:
$$\transl{ \Gamma   \vdash  M :  \tau }^{c, o} := \Typing {\InputII c {\vec k \in \ValueType { \Gamma }} {\Naming c {\vec x}.\, \transl { \Gamma   \vdash  M :  \tau }^o_{\vec k}}} {c: \otimes  \Gamma , o: \transl  \tau }.$$

The translation of terms is presented in
Figure~\ref{fig:translation-cbv-pcf}. Because the types in the context
are ensured to implement call-by-value, this translation is 
more involved than the previous ones, and has to be defined on the
typing relation instead of the terms themselves.
%
\begin{figure}
  \textbf{Translation of Terms}
  {\small
  \begin{align*}
    \transl{\Gamma  \vdash  \bot : A   }^{o}_{\vec k}
    &\quad\eqdef\quad
    \EmptyProcess
  \\
  \transl{\Gamma, x \vdash x :  \sigma  }^{o}_{\vec k}
    &\quad\eqdef\quad
                                               \Output o {k_x}.\, \Forwarder x o { \sigma /k_x}
  \\
  \transl{\Gamma \vdash \abs x M :  \sigma   \rightarrow   \tau }^{o}_{\vec k}
      &\quad\eqdef\quad
                                                           \AbsCbv o x { \sigma } {
                                                           (\transl { \Gamma , x :  \sigma   \vdash  M :  \tau }^o_{\vec k, x:v})_{v \in \ValueType { \sigma }}}
  \\
  \transl{\Gamma: \app{M}{N} : \tau}^{o}_{\vec k}
      &\quad\eqdef\quad
                                                      \AppCbv x { \sigma } o
                                                      {\transl M^{x}_{\vec k}}
                                                      {\transl N^o_{\vec k}}
                                                      \qquad ( \Gamma   \vdash  M :  \sigma )
  \\
  \transl{\Gamma \vdash \ifte M {N_1} {N_2} : \tau}^{o}_{\vec k}
        &\quad\eqdef\quad
        \shareInteract x y {\transl  \Gamma /\vec k}
        {\transl M^{x}_{\vec k}}
        {\InputII y {} {\ttrue: \transl {N_1}^o_{\vec k}; \ffalse: \transl {N_2}^o_{\vec k}}}
  \\
  \transl{\Gamma \vdash \mathsf{iszero}: \linlamNat \to \linlamBool}^o_{\vec k}
          &\quad\eqdef\quad
    \AbsCbv o x {\linlamNat} {\left ( 
    \begin{aligned}
      \Output o \ttrue \qquad \text{if n = 0}\\
      \Output o \ffalse \qquad \text{if n > 0}\\
    \end{aligned}\right)_{n \in  \mathbb{N} }}
  \\
  \transl{\Gamma \vdash \mathsf{succ}: \linlamNat \to \linlamNat}^{o}_{\vec k}
            &\quad\eqdef\quad
    \AbsCbv o x {\linlamNat} {\left( 
    {\Output o {n = 1}} \right)_{n \in  \mathbb{N} }
    } \\[-1em]
  \end{align*}
  }

  \textbf{Macros}
  
  {\footnotesize
  \[
  \begin{array}{rlll}
    \text{Name} & \text{Definition} & \text{Given}
    \\[1mm]
    \AbsCbv o x \sigma { (P_k) }
      &
           \Typing {\Output o \Lam.\, \Prom o r.\, \InputII r {}
        {k: \Naming r {x, o}.\, P_k}}
        {\Delta , o: \transl { \sigma   \rightarrow   \tau }}
        &
      \forall k, \Typing {P_k}{ \Delta , x: (\transl  \sigma /k)^\perp, o: \transl  \tau }
    \\[2mm]
    \UnLam x o v P
   & \Typing {\Split o {x, o} {
     \begin{aligned}
       &\quad \shareInteract x y {} {P[o := x]} {}\\
       &{\InputII y {} {\Lam: \Output {y^?} v.\, \Forwarder y o {}}}
     \end{aligned}}}
   {\Gamma , x: (\transl  \sigma /v)^\perp, o: \transl  \tau}& \Typing P { \Gamma , o : \transl{ \sigma   \rightarrow   \tau }}, v \in \ValueType { \sigma }
    \\[2mm]
    \AppCbv x  \sigma  o P Q
                & \Typing {\shareInteract x y { \Delta } Q
                  {\InputII y {v \in \ValueType{ \sigma }} {v.\, \UnLam y o v P}}}
   {\wn  \Delta , o: \transl  \tau}
   & \Typing Q {o: \transl { \sigma \to  \tau }, \wn  \Delta },\\
  &&   \Typing P {x: \transl { \sigma }, \wn  \Delta } 
  \end{array}
\]}
  
  \caption{Translation from call-by-value $ \lambda $-calculus to $\PILL$} 
  \label{fig:translation-cbv-pcf}
\end{figure}

\subsubsection{Soundness}

%
In the semantics, values can be recognised by the fact that they start
by sending an initial move on $o$.
%
\begin{restatable}{lemma}{valueChar}\label{lemma:valueChar}
  If a term $ \Gamma   \vdash  M :  \tau $ is a value, then its translation is of the
  form:
  $\transl M ^{o}_{\vec k} \similarProcesses \Output o \ell. P_{\vec
    k}$ for some $\ell  \in  \ValueType  \tau $.
\end{restatable}
%
For example, closed values of type $\mathbb{N}$ are in bijection with natural numbers.

\begin{restatable}{lemma}{subCbv}\label{lemma:subCbv}
  The effect of substitution of values on the translation is the following:
  \[
    \transl{\Gamma \vdash M \subst x N}^{o}_{\vec k} =
    \shareInteract y x {\transl  \Gamma  / \vec k}
    {
      P_{\vec k}
    }
    {
      \transl{\Gamma \vdash M}^{o}_{\vec k, x: \ell}
    }.
  \]
  where $N$ is assumed to be a value with
  $\transl N^{y}_{\vec k} = \Output y \ell. P_{\vec k}$.
\end{restatable}

We then deduce soundness and adequacy (however, in this setting
without recursion, adequacy is a much weaker result):
\begin{restatable}[Soundness and adequacy]{proposition}{cbvSound}
  Given two terms $ \Gamma \vdash M, N : \tau$, if $M  \rightarrow _{v} N$, then
  $\transl M^{c,o} \similarProcesses \transl N^{c,o}$. Moreover, if
  $ \llbracket M \rrbracket \similarProcesses  \llbracket n \rrbracket$ for $ \vdash  M :  \mathbb{N} $, then
  $M  \rightarrow _{v} n$.
\end{restatable}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> figures/meta_op.tex <==
\begin{figure}
  \small
  \boxit[Communications]{
    \begin{mathpar}
      \inferruleR[\rulename{com}]
      {\CCut a b {(\CSelect a k \PatternVar P \CFork
          {\CBranching b {i \in I} {\CBranch i {\PatternVar_i} {Q_i}}})}
        \Red
        \CCut {\PatternVar} {\PatternVari_k}
        {(P \CFork Q_k)}} {k \in I}
      \and
      \inferruleR[\rulename{rep}]
      {\CCut a b {(\CDer a \PatternVar P \CFork \CProm b \PatternVari Q \CFork R)}
        \Red
        \CCut a b {(R \CFork \CProm b q Q \CFork \CCut {\PatternVar} {\PatternVari} {(P \parallel Q)})}}
      {\ }
      \and
      \inferruleR[\rulename{nd}]
      {\CCut a b {(\CDer a \PatternVar P \CFork \CCoder b \PatternVari Q \CFork R)}
        \Red
        \CCut a b {(R \CFork \CCut {\PatternVar} {\PatternVari} {(P \parallel Q)})}}
      {\ }
    \end{mathpar}
  }
  \boxit[Reduction under context] {
    \begin{mathpar}
    \inferruleR[\rulename{par}]
    {P \CFork Q  \Red  P' \CFork Q}
    {P  \Red  P'}
    \
    \inferruleR[\rulename{par}]
    {\CCut a b P  \Red  \CCut a b {P'}}
    {P  \Red  P'}
    \
    \inferruleR[\rulename{cnx}]
    {\mathfrak a^+[P] \Red  \mathfrak a^+[P]}
    {P  \Red  P'}
    \
    \inferruleR[\rulename{str}]
    {P  \Red  Q'}
    {P \equiv P'  \Red Q  \equiv Q'}
  \end{mathpar}
  }
\caption{\label{sec:calc:opsem}Operational semantics of the calculus.}
\end{figure}


==> figures/ml_nd_op.tex <==

\begin{figure}
\boxit{
\begin{mathpar}
  \inferruleR[\rulename{race}]{\CCut a b {(\CDer a \PatternVar P \CFork \CCoder b \PatternVari Q \CFork R)} \rightarrow \CCut a b {(R \CFork \CCut {\PatternVar} {\PatternVari} {(P \parallel Q)})}}{\ }\\
    \inferruleR[\rulename{cxt}]{E[P]  \rightarrow  E[Q]} {P \rightarrow Q}
    \quad \quad  
    \inferruleR[\rulename{str}]{P  \rightarrow  Q} {P'\equiv P  \rightarrow 
      Q\equiv Q'}
\end{mathpar}
}
\caption{Operational semantics for $\MetalanguageName$}
\label{fig:ml_op}
\end{figure}


==> lindet.tex <==
% ! TEX root = main.tex
We start by showcasing our methodology in the simplest case:
\emph{deterministic} and \emph{linear} computation, using the setting
of \cite{lics11}. In this setting, both games and strategies are
represented as \textbf{event structures}, a causal model of concurrent
and nondeterministic computation. We offer a brief reminder on them in
\S~\ref{sec:es} before defining games and strategies in
\S~\ref{sec:games}. In \S~\ref{sec:lindet}, we recall the categorical
structure of strategies, and in particular \textbf{composition}. In
\S~\ref{sec:mall}, we offer our first contribution, which is a dialect
of the $ \pi $-calculus describing syntactically $\LinDet$: games are
described by session types and strategies by processes. In
\S~\ref{sec:interpretationLindet}, we show how the traditional
interpretation of the linear $ \lambda $-calculus can be factored through our
syntactc description.

\subsection{Event Structures}\label{sec:es}
Event structures were introduced by \cite{eventstructures} to give a
semantic model of causal concurrency (or true concurrency). From this
viewpoint, a system is a set of events along with a partial order
describing the \textbf{causal relationship} between events; and a
binary relation describing \textbf{conflict} (or incompatibility)
between events, ie. those events that cannot occur together in the
same run of the system. As a result, event structures model the system
\textbf{globally} rather than describe its executions.

We use here \emph{prime event structures with binary conflict}.

\begin{definition}
An ""event structure"" is a triple $(E,  \leq _E, \#)$ where $(E,  \leq _E)$ is
  a partial order, and $\# \subseteq E^2$ is a binary irreflexive relation satisfying: (1) 
%  \begin{enumerate}
%  \item 
$[e] \eqdef \{ e'  \in  E \mid e'  \leq  e\}$ is finite; and 
%  \item 
(2) if $e \# e'$ and $e'  \leq  e''$ then $e \# e''$.
%\end{enumerate}
\end{definition}
Two events $e,e'$ are in ""conflict"" when $e \# e'$ and are
""compatible"" otherwise.  Two compatible events which are not ordered
are called ""concurrent"". We write $e \imdep e'$ (""immediate causal
dependency"") when $e <_E e'$ with no events in between, and
$e \minconflict e'$ (""minimal conflict"") when $(e, e')$ is the only
conflicting pair in $[e] \cup [e']$. From $\imdep$ and $\minconflict$,
we can recover $ \leq $ and $\#$ via axiom (2). Depictions of "event
structures" will use $\imdep$ and $\minconflict$.

A notion of partial execution can be recoverd on event structures
through the notion of configuration.  Given an "event structure" $E$,
a ""configuration"" of $E$ is a subset $x \subseteq E$ down-closed for
$ \leq _E$ and conflict-free. We write $\config (E)$ for the set of
finite configurations of $E$. For $x \in \config (E)$, an
""extension"" of $x$ is an event $e \in E \setminus x$ such that
$x \cup \{e\} \in \config (E)$; we write $x \longcov e$.

An event structure $E$ is ""confusion-free"" when (1)
$e \minconflict e'$ implies $[e) = [e')$ and (2) the relation
$(\minconflict_E\, \cup\, =_E)$ is an equivalence relation. Its
equivalence classes are called ""cells"". Confusion-free event
structure have \textbf{local} nondeterminism and cells represent
choices between different branches of the program.

Finally, given a set $V \subseteq E$, the ""projection"" of $E$ to $V$
is the event structure $(V,  \leq _E \cap V^2, \# \cap V^2)$. 

\subsubsection*{Constructions on Event Structures} Given a family of event
structures $(E_{i \in I})$ we define their ""parallel composition"" $ \parallel
_{i \in I} E_i$ as follows. Its events are pairs $(i \in I, e \in
E_i)$. Causality and conflict are obtained by lifting those from the $E_i$:
\[
  (i, e)  \leq _{ \parallel _{E_i}} (j, e') \eqdef (i = j \wedge e  \leq _{A_i}
  e') \qquad(i, e) \#_{ \parallel _{E_i}} (j, e') \eqdef (i = j \wedge e \#_{A_i}
  e')
\]
%
Similarly, the ""nondeterministic sum"" of the $E_i$, written
$\sum_{i \in I} E_i$ has the same components as
$ \parallel _{i \in I} E_i$ except for conflict:
\[
  (i, e) \#_{\sum_{i \in I} E_i} (j, e') \eqdef (i = j  \Rightarrow  e \#_{E_i} e').
\]
%
The empty event structure, written $\intro*{\EmptyES}$ is the unit for
both parallel composition and sum.



\subsubsection*{Maps of Event Structures} It is customary to compare
concurrent systems using simulation. In event structures, this can be
done via maps between event structures. A ""partial map of event
structures"" is a partial function $f : E \rightharpoonup F$ such that
the direct image of a configuration is a configuration and which is
""locally injective@local injectivity"": $f$ restricted to any
configuration of $E$ is injective. We write $\intro*{\dom f}$ for the
domain of $f$. When $\dom f = E$, $f$ is said to be ""total@total
map"". A map represents a simulation of $E$ by $F$. Event structures
and total maps form a category $\intro*{\ES}$.

\subsection{Games and Strategies on Event Structures}\label{sec:games}
We recall the game model based on event structures
\cite{lics11}.
\subsubsection*{Games as Polarised Event Structures} 
\begin{figure}
  \centering
  \small
  \scalebox{1}{
  \subcaptionbox{\label{fig:unit->unit (CBV)}$\mathsf{unit}  \Rightarrow  \mathsf{unit}$ (CBV)}{
    \begin{tikzpicture}  

      \matrix [diag, column sep=0, row sep=0.2cm] {
        \textsf{unit}\&  \Rightarrow  \&\textsf{unit} \\[-2mm]
        \& |(l)| \Pla{\textsf{lam}} \\
        |(call)| \Opp {\textsf{call}} \\
        \& \& |(ret)| \Pla {\textsf{ret}}\\
      };
      \path[cause] (l) edge (call) (call) edge (ret);
    \end{tikzpicture}\ 
    \vspace{0.4em}
  }}\quad
\scalebox{1}{
  \subcaptionbox{\label{fig:unit->unit (CBN)}$\mathsf{unit} \Rightarrow \mathsf{unit}  \Rightarrow  \mathsf{unit}$ (CBN)}{
    \begin{tikzpicture}
      \matrix [diag, column sep=0, row sep=0.2cm] {
        \textsf{unit}\&  \Rightarrow \& \textsf{unit}\&  \Rightarrow  \&\textsf{unit} \\[-2mm]
        \& \& \& \& |(call)| \Opp{\textsf{call}} \\
        |(call')| \Pla{\textsf{call}}\& \& |(call'')| \Pla{\textsf{call}}\& \& |(ret)| \Pla{\textsf{ret}}\\ \\
        |(ret')| \Opp{\textsf{ret}} \& \& |(ret'')| \Opp{\textsf{ret}}\\
      };
      \path[cause] (call) edge (call') (call) edge (call'') (call') edge (ret') (call) edge (ret) (call'') edge (ret'');
    \end{tikzpicture}\qquad
    
  }}\ 
\scalebox{1}{
  \subcaptionbox{\label{fig:bool->bool (CBN)}$\mathsf{bool}
    \Rightarrow  \mathsf{bool}$ (CBN)}{
    \begin{tikzpicture}
      \matrix [diag, column sep=0.0cm, row sep=0.2cm] {
        \& |(n)| \vphantom{bool}\&\&  \&  \&|(n')| \vphantom{bool}\\[-2mm]
        \& \& \& \& \& |(c)| \Opp{\textsf{call}} \\
        \& |(c')| \Pla{\textsf{call}} \& \& \& |(retff')| \Pla {\textsf{ret}_{\ffalse}} \& \& |(rettt')| \Pla {\textsf{ret}_{\ttrue}} \\
        |(retff)| \Opp {\textsf{ret}_{\ffalse}}\& \&  |(rettt)| \Opp {\textsf{ret}_{\ttrue}} \&\\
      };
      \path[cause]
      (c) edge (c') (c') edge (retff) (c') edge (rettt) (c) edge (retff') (c) edge (rettt');
      \path (retff) edge[conflict] (rettt)
      (retff') edge[conflict] (rettt');
      \node at (n) { \textsf{bool} };
      \node at (n') { \textsf{bool} };
      \node at ($(n)!0.5!(n')+(0,-0.05)$) { $\Rightarrow$ };
    \end{tikzpicture}
    \vspace{0.3em}
  }}
  \caption{Examples of Games} 
 \label{fig:examples of games}
\end{figure}
As discussed in the introduction, a game is a set of moves plus some
extra structure encoding the rules of the game. These rules can be
adequately represented using an event structure:
\begin{definition}
  A ""game"" is an event structure $A$ along with a labelling
  $\pol : A  \rightarrow  \{\Neg -, \Pos +\}$ such that:
  \begin{enumerate}
  \item $A$ is "confusion-free" and ""race-free"": if $a \minconflict_A a'$, then $\pol(a) = \pol(a')$
  \item $(A,  \leq _A)$ is a ""forest"": elements of $[a]$ are totally ordered
    by $ \leq _A$ for any $a  \in  A$.
  \end{enumerate}
\end{definition}
These restrictions on games make the development simpler and is
sufficiently expressive to represent the behaviour of types we are
interested in. Configurations of a game represent \textbf{valid plays}
of the game, respecting the rules of the game. Parallel composition
and nondeterministic sum extend to games. Similarly, the empty event
structure extends to the empty game written $\intro*{\EmptyGame}$.
Given a "game" $A$, its ""dual"" $A^\perp$ is the game obtained from
$A$ by reversing polarities. Given an element $e \not\in A$ and a
polarity $p \in \{-, +\}$, we write $e^p \cdot A$ (""lifting"") the
game obtained from $A$ by adjoining an event $e$ with polarity $p$
which is below and consistent with all events of $A$. If
$x, y \in \config (A)$, we write $x \subseteq^p y$ for $x \subseteq y$
and $\pol(y \setminus x) \subseteq \{p\}$.
%
A game is ""negative@negative game"" when its minimal events are all
negative; ""positive@positive game"" if they are all positive. A game
is ""polarised"" if it is either negative or positive.



We give a few examples of games in Figure \ref{fig:examples of
  games}. Each game corresponds to a particular function type, under a
particular calling convention (call-by-name or
call-by-value). Remember that a game represents the allowed messages
that Program and Context can exchange during the course of the
execution. As depicted in Figure \ref{fig:unit->unit (CBV)}, in
$\UnitType \rightarrow \UnitType$ in call-by-value, there are three
moves. The first move is a Player move telling the context that the
program has evaluated to a closure (as it may diverge). Once this move
has been received, Context can call the closure via
\textsf{call}. When called, Program can return from the closure via
\textsf{ret}. The only rules we have here are due to the causal
ordering which constrains the order in which the moves can be played
by the players. In call-by-name, however, the dynamic is reversed:
Context starts the computation by calling the function\footnote{There
  is no need for Program to tell Context it has evaluated to a closure
  since $ \lambda x.\, \bot \equiv \bot$ in call-by-name, while this
  equality does not hold in call-by-value}. Moreover, arguments are
not values but \emph{thunks}. Each thunk can be evaluated by Program
via a \textsf{call} move, as illustrated in Figure~\ref{fig:unit->unit
  (CBN)}. Finally, our third example illustrates the interpretation of
types with several values: each value becomes a different
move. Because there can only be one value exchanged in one run of the system,
the different moves are in conflict as evidenced in Figure~\ref{fig:bool->bool
(CBN)}. Note that moves are drawn in columns, to ease readability.

\subsubsection*{Strategies as Labelled Event Structures} A strategy
will represent a concurrent program so it will be an event structure
$S$. The fact that a strategy $S$ plays on a game $A$ (ie. respects
the rules of $A$) is formalising by requiring a map $S \rightarrow A$.
Strategies will be their own event structure $S$ along with a
labelling map $S \rightarrow A$. Often the labelling will be
injective, allowing us to see $S$ as a subset of $A$; but this is not
always the case (cf. Figure~\ref{fig:non injective strategy}).
\begin{definition}
  A ""deterministic strategy"" (in the rest of the text, simply "strategy") on a "game" $A$ is a "total map of event structures" $ \sigma : S   \rightarrow   A$ such that
  \begin{description}
  \item [Receptivity] For $x \in \config (S)$ and $a$ a negative
    extension of $ \sigma \, x$, there exists a unique $x \longcov s$ with
    $ \sigma \, s = a$.
  \item[Courtesy] For any $s  \imdep _S \, s'$ such that $ \sigma \, s$ and $ \sigma \, s'$
    are concurrent, $\pol(s) = -$ and $\pol(s') = +$.
  \item[Determinism] If $s \minconflict_S\, s'$, then
    $ \sigma \, s \minconflict_A\, \sigma \, s'$ and both are negative.
  \end{description}
\end{definition}
Asking for $ \sigma $ to be a map of event structures amounts to
asking that $ \sigma $ respects the rules of the game: configurations
of $S$ should correspond to configurations (ie. executions) of $A$, in
particular $ \sigma $ should not be able to play a move before it has
played the move unlocking it. Moreover, within a configuration, moves
should be played at most once. The conditions of receptivity and
courtesy are needed for strategies to form a category and imply a
strong form of asynchrony (see \S~\ref{sec:compStrat}). Determinism
amounts to saying that nondeterministic choices can only come from
Context. From $A$, $ \sigma $ imports a notion of polarity on the events of
$S$.

A strategy from a game $A$ to a game $B$ is a strategy on the
composite game $A^\perp \parallel B$. We write $ \sigma : A \profto B$
to distinguish them from maps. We will omit displaying both $S$ and
$A$, along with the labelling, but rather adopt a concise
representation as in Figure \ref{fig:examples of strategies} where we
only display $S$ with labels in $A$ and use columns to
disambiguate. Figure~\ref{fig:parallel} depicts a simple example of a
concurrent strategy, which given two thunks evaluates them in parallel
and only returns when both have returned. We have highlighted in blue
the causal links that the strategy adds onto the game, which must be
from negative to positive by courtesy. Figure~\ref{fig:non injective
  strategy} depicts a strategy where the labelling $ \sigma $ is not
injective. Indeed, the event $\mathsf{ret}_{\ttrue}$ occurs twice, but
the two occurrences are in conflict (inherited from the conflict
$\Opp{\mathsf{ret}_{\ttrue}} \minconflit
\Opp{\mathsf{ret}_{\ffalse}}$).

\begin{figure}\small
  \subcaptionbox{\label{fig:parallel}Interpretation of $ \lambda x y.\, x  \parallel  y$ (CBN)}{
    \begin{tikzpicture}
      \matrix[diag, column sep=0cm] {
        |(aa)| \mathsf{unit} \&\  \Rightarrow\  \& |(b)| \mathsf{unit}\& \ \Rightarrow\  \& |(c)| \mathsf{unit} \\[-2mm]
        \&\&\& \& |(q)| \Opp{\textsf{call}} \\
        |(q1)| \Pla{\textsf{call}} \& \& |(q2)| \Pla{\textsf{call}} \\
        |(a1)| \Opp{\textsf{ret}} \& \& |(a2)| \Opp{\textsf{ret}} \\
        \& \& \& \& |(a)| \Pla{\textsf{ret}} \\
      };
      \path[cause]
      (q) edge (q1)
      (q) edge (q2)
      (q1) edge (a1) (q2) edge (a2)
      (a1) edge[color=blue!80!black] (a)
      (a2) edge[color=blue!80!black] (a);
      \node at (aa) {$$};
      \node at (b) {$\mathsf{unit}$};
      \node at (c) {$ \mathsf{unit}$};
    \end{tikzpicture}\qquad
    \vspace{0.5em}
    }
    \qquad
  \subcaptionbox{\label{fig:non injective strategy} Interpretation of $ \lambda x.\, \ifSyntax
    {x} \ttrue \ttrue : \mathbf{bool}$ (CBN)}{
  \begin{tikzpicture}
    \matrix[diag, column sep=0.cm] {
      \& \textsf{bool} \& \& \Rightarrow \& \& \textsf{bool} \\[-2mm]
      \& \& \& \& \& |(c)| \Opp{\textsf{call}} \\
      \& |(c')| \Pla{\textsf{call}} \\
      |(fs)| \Opp{\textsf{ret}_{\ffalse}} \& \& |(ts)| \Opp{\textsf{ret}_{\ttrue}} \\
      \& \& \& \& |(fs')| \Pla{\textsf{ret}_{\ttrue}} \& \& |(ts')| \Pla{\textsf{ret}_{\ttrue}}\\
    };
    \path[cause]
    (c) edge (c') (c') edge (fs) (c') edge (ts)
    (fs) edge[color=blue!80!black] (fs') (ts) edge[color=blue!80!black] (ts');
    \path (fs) edge[conflict] (ts);
 
  \end{tikzpicture}
}
\caption{\label{fig:examples of strategies}Examples of Strategies}

\end{figure}

Given a "game" $A$, we form the ""copycat strategy"" on $A$,
$\cc_A : \CC_A \rightarrow A^\perp \parallel A$, as follows. The
events of $\CC_A$ are exactly those of $A^\perp \parallel A$, and
$ \leq _{\CC_A}$ is obtained from the transitive closure of
$ \leq _{A^\perp \parallel A} \cup \{ (a, \bar a) \mid a \in A^\perp
\parallel A\text{ is negative}\}$ where we write
$\bar a \in A^\perp \parallel A$ for the corresponding event to $a$ on
the other side. Then $a \#_{\CC_A} a'$ holds when
$[a]_{\CC_A} \cup [a']_{\CC_A} \in \config (A^\perp \parallel A)$. The
labelling function $\cc_A$ is simply the identity. A strategy is
""negative@negative strategy"" when its minimal events are all
negative. Copycat for example is a negative strategy.

The empty strategy $\intro*{\weakening A}$ on a game $A$ is defined as
the inclusion $A_0 \subseteq A$ where $A_0$ contains events $a \in A$
such that $[a]$ only contains negative events (ie. it is the minimal
receptive strategy).

Because $S$ is arbitrary, equality of strategies is not
meaningful. Rather, we consider strategy up to isomorphism. Two strategies
$ \sigma : S \rightharpoonup A$ and $ \tau : T \rightharpoonup A$ are
""isomorphic"" (written $ \sigma \cong \tau $) when there exists an
isomorphism of event structures $ \varphi : S \cong T$ (that is a map
$S \to T$ with an inverse) such that
$ \tau \circ \varphi = \sigma $.

\subsection{The category $\LinDet$}\label{sec:lindet}
We now explore the algebraic properties of strategies, which have
guided the choice for the metalanguage $\PIMALL$ (introduced in
\S~\ref{sec:mall}).
\subsubsection*{Composition of Strategies}\label{sec:compStrat}
Let us first review the main operation on strategies: composition.
%
Given a strategy $ \sigma  : A \profto B$ from $A$ to $B$, and a strategy $ \tau  : B \profto C$
from $B$ to $C$, we would like to combine them to form a strategy
$ \tau   \odot   \sigma $ from $A$ to $C$. This is done by letting $ \sigma $ and $ \tau $ interact
on $B$, giving an event structure $T  \circledast  S$ (not a strategy) which
projects to $A  \parallel  B  \parallel  C$. The composition is then obtained by hiding
events projected to $B$ to recover a strategy $ \tau   \odot   \sigma  : A^\perp  \parallel  C$.

In the world of traces, interaction is usually obtained as the
intersection of compatible traces -- ie. traces whose behaviour on
$A^\perp  \parallel  B$ and $B^\perp  \parallel  C$ belong to $ \sigma $ and $ \tau $ respectively. In
our causal setting, this is a bit more complex than a mere intersecton
since causal constraints from $ \sigma $ and $ \tau $ must be merged. In event
structure, this operation can be elegantly represented by a
pullback. From \cite{eventstructures} we know that $\ES$ has all
pullbacks.

The interaction
$ \tau \circledast \sigma : T \circledast S \rightarrow A \parallel B
\parallel C$ of $ \sigma : S \rightarrow A^\perp \parallel B$ and
$ \tau : T \rightarrow B^\perp \parallel C$ is obtained as the
pullback of
$ \sigma \parallel C : S \parallel C \rightarrow A \parallel B
\parallel C$ and of
$A \parallel \tau : A \parallel T \rightarrow A \parallel B \parallel
C$. Their ""composition"" is then obtained by "projecting@projection"
$T \circledast S$ to events that are sent to $A$ or $C$:
$$T  \odot  S = (T  \circledast  S)  \downarrow  \{ e  \in  T  \circledast  S \mid ( \tau   \circledast   \sigma )(e) \in A  \parallel  C \} \qquad  \tau   \odot   \sigma  =  \tau   \circledast   \sigma  \vert_{T  \odot  S} : T  \odot  S  \rightarrow  A^\perp  \parallel  C.$$

\begin{lemma}[\cite{lics11}]
  "Composition" of strategies is associative, and "copycat" is an
  identity on "strategies", both up to isomorphism.
\end{lemma}
For copycat to be an identity, the conditions of receptivity and
courtesy are necessary. Intuitively, this is because composing a
strategy with copycat amounts to prefixing it with an asynchronous
buffer; and if the strategy is too ``synchronous'', this buffer may
have observable effects. 

\subsubsection{Categorical Structure}\label{sec:lindet cat} We define $\intro*{\LinDet}$, the category
whose objects are finite "games" and morphisms from $A$ to $B$ are
"strategies" $ \sigma : A \profto B$. First, duality of games extends
to an isomorphism of category $\LinDet \cong \LinDet^{\text{op}}$: any
strategy $ \sigma : A \profto B$ can be regarded as a strategy
$ \sigma ^\perp : B^\perp \profto A^\perp$. Moreover, parallel
composition of games forms a monoidal structure on
$\LinDet$. Therefore, $\LinDet$ is compact-closed:
\begin{lemma}[\cite{cg1}]
  $(\LinDet,  \parallel , \EmptyGame, (-)^\perp)$ is a compact-closed category.
\end{lemma}

\noindent There is a way to lift certain maps of event structures between games to
strategies that is useful to obtain structural maps. A ""map of games"" is a
partial map $f : A \rightharpoonup B$ preserving polarities such that (1) $f$
restricted to its domain is bijective, (2) $f$ preserves causal ordering and
conflict. The ""lifting of $f$@lifting of maps"" is the strategy $\Lift f \eqdef
\CC_A \downarrow A^\perp \parallel \dom f \xrightarrow{A^\perp \parallel
f}A^\perp \parallel B$.
%
Though $\LinDet$ does not have (co)products, it has weak (co)products, that are
defined by lifting. Given two games $A$ and $B$, let us define $A \with B \eqdef
(\Left^- \cdot A) + (\Right^- \cdot B)$. There are
obvious "maps of games" $p_1 : A \with B \rightharpoonup A$ and
$p_2 : A \with B \rightharpoonup B$ and we let
$ \pi _1 = \Lift {p_1} : A \with B \profto A$ and
$ \pi _2 = \Lift {p_2} : A \with B \profto B$.

\begin{restatable}{lemma}{productLinDet}\label{lemma:product}
  For every strategies $ \sigma : A \profto B$ and
  $ \tau : A \profto C$ there exists a strategy
  $ \intro*{\Pairing {\sigma , \tau}} : A \profto B \with C$ such that
  $ \pi _1  \odot   \Pairing {\sigma ,  \tau}  \cong    \sigma$  and  $\pi _2  \odot  \Pairing {\sigma ,  \tau}   \cong   \tau$ .
  %
  By duality, we obtain weak coproducts $A  \oplus  B = (A^\perp \with B^\perp)^\perp$.
\end{restatable}

\subsection{A Metalanguage for $\LinDet$: $\PIMALL$}\label{sec:mall}
In this section, we show how to use a session $ \pi $-calculus to
represent games and strategies of $\LinDet$.

\subsubsection*{Games as Session Types.} Games can easily be seen as
protocols from the point of view of Program: positive moves are
outputs and negative moves inputs. It turns out that all finite games
can be easily described by $ \parallel $, $\oplus$ and $\with$ and prefixing which are all
standard operation both in Session Types and in Linear Logic.

This suggests the following grammar for session types corresponding to
games:
$$T \Coloneqq (T \CPar  \ldots  \CPar T) \mid \CWith {i \in I} {T_i} \mid \CPlus {i \in I} {T_i}.$$
%
In the grammar, $k$, $i$ and $j$ range over \emph{labels} $\mathbb L$,
to be thought of as values such as integers and booleans.  The type
grammar corresponds to Multiplicative Additive Linear Logic (without
additive units and literals) except that $ \otimes $ and $\parr$ have
been collapsed into one operation, $\parallel$ (similarly for the
multiplicative units). This is to be expected since the main asymmetry
between $\otimes$ and $\parr$ arise as a way to avoid deadlocks during
cut-elimination. In our setting, deadlocks are permitted so there is
no need for a distinction. We call this variant \emph{compact-closed
  MALL}, because identifying $\otimes$ with $\parr$ is a common
feature in models that are compact-closed (eg. games or the relational
model).

Types come equipped with a notion of \emph{duality} stemming from the usual
De Morgan laws: $\with$ and $\oplus$ are dual to each other and
$ \parallel $ and $\EmptyType$ are self-dual. We will use the notation
$\ell^- \cdot T$ and $\ell^+ \cdot T$ for $\with_{i \in \{\ell\}} T$
and $\oplus_{i \in \{\ell\}} T$. We will also use the binary version
$A \with B$ for $\with_{\ell \in \{\Inl, \Inr\}} T_\ell$ with
$T_\Inl = A$ and $T_\Inr = B$; and dually for $A \oplus B$. For instance,
let us introduce
$\mathbb B = \Start^- \cdot (\oplus_{b \in \{\ttrue, \ffalse\}} 1)$, the type of
(call-by-name) booleans. The initial move represents the evaluation
request from Context, as call-by-name booleans are thunks waiting for
a request from the environment before starting to evaluate.

\subsubsection{Strategies as Processes.} We show now how to describe
strategies with processes whose actions represent events of the
strategy. An action is composed of a channel name; telling us which
"cell" of the game we play, and a payload (ie. a value) indicating
which event inside the cell is played. In the case of the
$ \lambda $-calculus, the channel indicates for instance which external
function we call, and the payload which value it is called
with.

However, there is more: playing a move $a \in A$ unlocks new moves
(the successors of $a$ in $A$), which in this setting means that new
channels are available to denote the successor. That means that for
instance a positive action will have the shape
$\CPositiveAction a v {\vec x}$ where $a$ is a channel; $v$ the
payload and $\vec x$ a list of channels corresponding to the
successors of $a$ in the game.

The grammar for processes is defined as follows:
$$
\begin{aligned}
  P, Q ::= \, &\CZero \mid P \CFork Q  \mid \CCut a b P
  \mid \CBranching c {i \in i} {\CBranch i {\vec x_i} P_i}  \mid \CSelect c k {\vec x} P\\
\end{aligned}$$

\subsubsection{Typing rules} We now describe the typing rules for the
calculus. Typing contexts are of the form
$a_1: A_1, \ldots , a_n: A_n$ where each $A_i$ is a rooted type. While
typing judgements are flat lists, games have more structure since
$(A  \parallel  B)  \parallel  C$ is \emph{only} isomorphic to $A  \parallel  (B  \parallel  C)$; not
equal. This prompts us to define an adequation relation between
contexts non-rooted type follows:
$$
\ContextElaboration {x} T = x: T \quad \text{(when $T$ is rooted)} \qquad
\ContextElaboration {\vec x, \vec y} {T  \parallel  U} = \ContextElaboration {\vec x} T, \ContextElaboration {\vec y} U.
$$ and undefined otherwise. Note that for the second equation, the decomposition in $\vec x, \vec y$ of any list $\vec z$ is unique, given $T  \parallel  U$. Typing judgements are simply of the
form $\Typing P {\Gamma}$. The rules are described in Figure
\ref{fig:mall typing}. When writing down processes, we often emit the
list of successors $\vec x$. This can mean two things: if the move is
maximal, it has no successors, and we omit the empty list
$ \epsilon $; or the move has a unique successor and we use the
standard convention of session types to re-use the same name:
eg. $\CPositiveActionS a k$ for $\CPositiveAction a k a$.


\begin{figure}
  \boxit {
    \begin{mathpar}
      \infer{\Typing \CZero { \Gamma }} {\ } \and
      \infer
      {\Typing  {P \CFork Q}{ \Gamma_1,  \Gamma _2}}
      {\Typing {P}{ \Gamma _1} \and \Typing  {Q} { \Gamma _2}}
      \and
      \infer
      {\Typing  {\CCut a b P}{ \Gamma }}
      {\Typing  {P}{ \Gamma , a: A, b: A^\perp}}
      \and
      \infer
      {\Typing {\CBranching a {i \in I} {\CBranch i {\PatternVar_i} {P_i}}}{ \Gamma, a: \CWith {i \in I} {T_i} }}
      {\forall i \in I, \Typing  {P_i}{ \Gamma, \ContextElaboration {\PatternVar_i} T_i}}
      \and
      \infer
      {\Typing {\CSelect a k \PatternVar P}{ \Gamma, a: \CPlus {i \in I} {T_i} }}
      {k\in I \and \Typing  {P_i}{\Gamma, \ContextElaboration \PatternVar T_k}}
    \end{mathpar}
  }
  \caption{\label{fig:mall typing}Typing rules of the calculus}
\end{figure}


An example of a useful process is the ""forwarder@fw""
$\Typing {\Forwarder a b A} {a: A, b: A^\perp}$, the syntactic counterpart
to the "copycat strategy". It is defined by induction on a rooted type $A$:
$$
\begin{aligned}
  \Forwarder a b {\EmptyType} &\eqdef \CZero &
  \Forwarder a b {T^\perp} &\eqdef \Forwarder b a {T}
  \\
  \Forwarder a b {\with_{i \in I} (T^1_i  \parallel   \ldots   \parallel  T^{n_i}_i)}
  &\eqdef \CBranching a {i \in I} {\CBranch i {a_1,  \ldots , a_n} {\CPositiveAction b i {b_1,  \ldots , b_{n_i}} { \parallel _{1  \leq  j  \leq  n_i} \Forwarder {a_j} {b_j} {T^j_i}}}}
  \\
\end{aligned}$$
\noindent Another more concrete example is the process \textsf{if} for call-by-name conditional:
$$\small\mathsf{if}^o \ {c} \ {b_1} 
\ {b_2} \eqdef \Typing {\InputII o {} {\Start: {\Output c \Start.\, c\with \left\{
  \begin{aligned}
    &\ttrue: \Output {b_1} \Start.\, \Forwarder {o} {b_1} {\mathbb B} \\
    &\ffalse: \Output {b_2} \Start.\, \Forwarder {o} {b_2} {\mathbb B} \\
  \end{aligned}\right. }}} {c : (\mathbb B)^\perp, b_i: (\mathbb B)^\perp, o: \mathbb B}$$
It has four channels: $c$ for the condition, $b_1$ and $b_2$ for the values of
the branches, and $o$ for the output. When Context requests the outcome of
$i$, the condition is evaluated, and, according to the value received, $b_1$ or
$b_2$ is evaluated and its answer is forwarded to $o$. 


\subsection{Interpretation into $\LinDet$}\label{sec:interpretationLindet}
The interpretation of $\PIMALL$ inside $\LinDet$ maps session types to
games; and processes to strategies. It follows the categorical
structure detailed in \ref{sec:lindet cat}.
\subsubsection*{Interpretation of Types} First, let us interpret types
as finite games as follows:
$$ \llbracket \EmptyType \rrbracket = \EmptyGame\qquad  \llbracket T_1  \parallel   \ldots   \parallel  T_n \rrbracket =  \llbracket T_1 \rrbracket  \parallel   \ldots   \parallel   \llbracket T_n \rrbracket \qquad  \llbracket \with_{i \in I} T_i \rrbracket = \with_{i \in I}  \llbracket T_i \rrbracket \qquad  \llbracket \oplus_{i \in I} T_i \rrbracket = \oplus_{i \in I}  \llbracket T_i \rrbracket.$$
We have $ \llbracket T^\perp \rrbracket =  \llbracket T \rrbracket^\perp$ as desired. Moreover, every game arises
as the interpretation of a type:
\begin{lemma}[\cite{POPL19}]
  For every finite game $A$, there exists a type $T$ such that
  $ \llbracket T \rrbracket  \cong  A$.
\end{lemma}
Contexts are likewise interpreted as the parallel composition of their
component:
$ \llbracket a_1:T_1, \ldots , a_n: T_n \rrbracket = \llbracket T_1
\rrbracket \parallel \ldots \parallel \llbracket T_n \rrbracket$.

\subsubsection*{Interpretation of Terms} We now interpret typing
derivations as morphisms in $\LinDet$.  The judgement
$\Typing P { \Delta }$ will be interpreted as a "strategy" on
$ \llbracket \Delta \rrbracket$. The interpretation is described in
Figure \ref{fig:interpMALL} where we use the fact that any strategy on
$ \llbracket  \Gamma , \ContextElaboration {\vec x} T \rrbracket$ can be viewed as a strategy
$ \llbracket  \Gamma  \rrbracket^\perp \profto  \llbracket T \rrbracket$ through basic associativity. This conversion
is left silent for ease of reading.

The interpretation of outputs and inputs is done using the weak product
structure. The interpretation of restriction uses the trace operator
induced by the compact-closed structure, which consists in composing
by copycat to connect $a$ and $b$ via an asynchronous forwarder.

Notice that
$ \llbracket \Forwarder a b T \rrbracket = \cc_{ \llbracket T
  \rrbracket}$ and that $ \llbracket ( \nu ab) (P \mid Q) \rrbracket$
where $a \in \fc P$ and $b \in \fc Q$ is equal to
$ \llbracket Q \rrbracket \odot \llbracket P \rrbracket$. 
%
\begin{figure}
\small
  \begin{mathpar}
 \left \llbracket
      \infer{\Typing \CZero  \Delta }{ }
    \right \rrbracket = \weakening  \Delta 
\quad
  \left\llbracket\vcenter{
  \infer{\Typing {P \CFork Q}{ \Gamma_1 ,  \Gamma_2}}
  {\Typing {P} {\Gamma_1} \qquad \Typing Q {\Gamma_2}}}
  \right\rrbracket =  \llbracket P \rrbracket  \parallel   \llbracket Q \rrbracket
\and
%
\left\llbracket\vcenter{\infer
  {\Typing {\CSelect a k {\vec x} P}{ \Gamma , a: \oplus_{i \in I} T_i}}
  {k \in I \and \Typing {P} { \Gamma , \ContextElaboration {\vec x}{T_k}}}}
\right\rrbracket
= ( \pi _k^\perp :  \llbracket T_k \rrbracket \profto  \llbracket \oplus_{i \in I} T_i \rrbracket) \odot ( \llbracket P \rrbracket :  \llbracket  \Gamma  \rrbracket^\perp \profto  \llbracket T_k \rrbracket)
  \and
  
  \left\llbracket\vcenter {
  \infer{\Typing {\CBranching a {i \in I} {\CBranch {i} {\vec x_i}{P_i}}}{ \Gamma , a: \with_{i \in I} T_i}}
  { \forall i: I, \Typing {P_i} { \Gamma , \ContextElaboration{\vec x} {T_i}}}}
\right\rrbracket = \Pairing { \llbracket P_i \rrbracket :  \llbracket  \Gamma  \rrbracket^\perp \profto  \llbracket T_i \rrbracket}_{i \in I}

  \and
  \left\llbracket\vcenter{
  \infer{\Typing{\cut a b T P} { \Gamma}}
  {\Typing {P} {a: T, b: T^\perp, \Gamma}}}
  \right\rrbracket = ( \llbracket P \rrbracket :  (\llbracket T \rrbracket^\perp  \parallel   \llbracket T \rrbracket) \profto  \llbracket  \Gamma  \rrbracket) \odot ("\cc_{ \llbracket T \rrbracket}@copycat strategy" : \emptyset \profto  \llbracket T \rrbracket  \parallel   \llbracket T \rrbracket^\perp)
  \end{mathpar}
  \caption[Interpretation]{Interpretation of $\PIMALL$ into $\LinDet$}
  \label{fig:interpMALL}
\end{figure}

Since strategies are finite, we have a definability result.
\begin{theorem}[Definability, \cite{POPL19}]
  Every "strategy" in $ \llbracket  \Delta  \rrbracket$ is the interpretation of a process
  $\Typing P  \Delta $.
\end{theorem}

\subsubsection*{Structural Congruence} Before describing the operational
semantics of this metalanguage, we start as usual by giving the
structural congruence on it.

Unlike more standard variants of the $ \pi $-calculus, this congruence
has to take into account the asynchronous permutations allowed by the
game semantics. We formalise them through the notion of
\textbf{prefix}. A prefix $\mathfrak a$ is a pair of an arity and a
context with as many holes as the arity. They are described by this
grammar:
$$
\begin{aligned}
  \mathfrak a ::= \CSelect a k \PatternVar [] 
\mid \CBranching a {i \in I} {\CBranch i {\PatternVar_i} {[]_i}} \\
\end{aligned}$$
The arity of all prefixes is one, except the branching prefix whose
arity is the indexing set. Given a prefix $\mathfrak a$ with arity
$I$, and a family of process $(P_i)_{i \in I}$, we write
$\mathfrak a[P_i]_{i \in I}$ for the substitution. A prefix is
positive (written $\mathfrak a^+$) when it is a dereliction or a
selection, empty otherwise. We also adopt the convention that a prefix
$\mathfrak a^p$ is a prefix of polarity $p$ on channel $a$.

We write $\BoundVars {\mathfrak a}$ for the set of variables occurring
in the pattern in $\mathfrak a$. Two prefixes $\mathfrak a$ and
$\mathfrak b$ are orthogonal, written $\mathfrak a \bot \mathfrak b$
when
$(\{a\} \cup \BoundVars {\mathfrak a}) \cap (\{b\} \cup \BoundVars
{\mathfrak b}) = \emptyset$.

The permutation rules are defined in Figure \ref{fig:calc:cong}.
\begin{figure}
  \boxit[$ \parallel $ is a monoid] {
    \begin{mathpar}
      \infer {P \CFork \CZero  \equiv  P} {\ } \and
      \infer {P \CFork Q  \equiv  Q \CFork P}{\ }  \and
      \infer {(P \CFork Q) \CFork R  \equiv  P \CFork (Q \CFork R)}{\ }  \and
    \end{mathpar}
  }
  \boxit[Basic properties of restriction] {
    \begin{mathpar}
      \infer {\CCut a b {\CZero}  \equiv  \CZero}{\ }  \and
      \infer {\CCut a b {P}  \equiv  \CCut b a P}{\ }  \and
      \infer {\CCut a b {\CCut c d P}  \equiv  \CCut c d {\CCut a b P}}{\{a, b\} \cap \{c, d\} = \emptyset}  \and
      \infer {\CCut a b {(P \CFork Q)}  \equiv  (\CCut a b P) \CFork Q}{\fv Q \cap \{a, b\} = \emptyset} \and
    \end{mathpar}
  }
  \boxit[Permutations of prefixes and cut] {
    \begin{mathpar}
      \infer {\CCut a b {\mathfrak a^-[P_i]_{i \in I}}  \equiv  \CZero}{\ } \and
      \infer {\CCut a b {\mathfrak c^+[P]}  \equiv  \mathfrak c^+[\CCut a b P]} {c \not\in \{a, b\}} \and
      \infer {\CCut a b {\mathfrak c^-[P_i]_{i \in I}}  \equiv  \mathfrak c^-[\CCut a b {P_i}]_{i \in i}} {c \not\in \{a, b\}} \and
      \infer {\CCut a b {(\mathfrak a^-[P_i]_{i \in I} \CFork \mathfrak c^-[Q_j]_{j \in J})}  \equiv  \mathfrak c^-[\CCut a b {(\mathfrak a^-[P_i]_{i \in I} \CFork Q_j)}]_{j \in J}}{c \not\in \{a, b\}} \and
    \end{mathpar}
  }
  \boxit[Permutation between prefixes] {
    \begin{mathpar}
      \infer{\mathfrak a^+[P] \CFork Q  \equiv  \mathfrak a^+[P \parallel Q]}{\BoundVars {\mathfrak a} \cap \fv Q = \emptyset}\and
      \infer{\mathfrak a^+[\mathfrak b^+[P]]  \equiv  \mathfrak b^+[\mathfrak a^+[P]]}{\mathfrak a \bot \mathfrak b }\and
      \infer{\mathfrak a^-[\mathfrak b^-[P_{ij}]_{j \in J}]_{i \in I}  \equiv  \mathfrak b^+[\mathfrak a^+[P_{ij}]_{i \in i}]_{j \in J}}{\mathfrak a \bot \mathfrak b}\and
    \end{mathpar}
  }
  \caption{\label{fig:calc:cong} Rules for the structural congruence}
\end{figure}

\begin{restatable}{lemma}{soundnessStructCong}
  Given $\Typing {P, Q} { \Gamma }$, if $P  \equiv  Q$ then $ \llbracket P \rrbracket  \cong   \llbracket Q \rrbracket$.
\end{restatable}

\subsubsection{Operational Semantics} Using the structural congruence,
we can now define the operational semantics of our calculus, written
$ \rightarrow _d$ (for deterministic) givne as follows:

The rules of the operational
semantics are given in Figure \ref{sec:calc:opsem}. In the reduction
under context, $ \alpha $ stands for either $d$ or $nd$.
\begin{figure}
  \boxit[Communication rules]{
    \begin{mathpar}
      \infer
      {\CCut a b {(\CSelect a k \PatternVar P \CFork
          {\CBranching b {i \in I} {\CBranch i {\PatternVar_i} {Q_i}}})}
        \DetRed
        \CCut {\PatternVar} {\PatternVari_k}
        {(P \CFork Q_k)}} {k \in I}
      \and
      \infer
      {\CCut a b {(\CDer a \PatternVar P \CFork \CProm b \PatternVari Q \CFork R)}
        \DetRed
        \CCut a b {(R \CFork \CProm b q Q \CFork \CCut {\PatternVar} {\PatternVari} {(P \parallel Q)})}}
      {\ }
      \and
      \infer
      {\CCut a b {(\CDer a \PatternVar P \CFork \CCoder b \PatternVari Q \CFork R)}
        \NDetRed
        \CCut a b {(R \CFork \CCut {\PatternVar} {\PatternVari} {(P \parallel Q)})}}
      {\ }
    \end{mathpar}
  }
  \boxit[Reduction under context] {
    \begin{mathpar}
    \infer
    {P \CFork Q  \rightarrow _ \alpha  P' \CFork Q}
    {P  \rightarrow _ \alpha  P'}
    \and
    \infer
    {\CCut a b P  \rightarrow _ \alpha  \CCut a b {P'}}
    {P  \rightarrow _ \alpha  P'}
    \and
    \infer
    {\mathfrak a^+[P]  \rightarrow _ \alpha  \mathfrak a^+[P]}
    {P  \rightarrow _ \alpha  P'}
    \and
    \infer
    {P  \rightarrow _ \alpha  Q'}
    {P \equiv P'  \rightarrow _ \alpha  Q  \equiv Q'}
  \end{mathpar}
  }
\caption{\label{sec:calc:opsem}Operational semantics of the calculus.}
\end{figure}




\subsection{Interpreting an Affine $ \lambda $-Calculus in
  $\LinDet$}\label{sec:affinelambda}
As the first example of our methodology, we show how to translate an
affine $ \lambda $-calculus into $\LinDet$, through a syntactic
translation into $\PIMALL$. The resulting model characterises
$ \beta \eta$-equivalence. Types of affine $ \lambda $-calculus are given by
the grammar: $\tau \Coloneqq \linlamBool \mid \tau \linto \tau$. The affine typing system has the following standard rules:
\[
\begin{array}{c}
\small
  \prftree
  {\Gamma, x:\tau_1 \vdash M:\tau_2}
  {\Gamma \vdash \abs x M : \tau_1 \linto \tau_2}
\quad
  \prftree
  {\begin{array}{l}
  {\Gamma \vdash M_1: \tau_1 \linto \tau_2}\\
  {\Delta \vdash M_2: \tau_1}
  \end{array}} 
  {\Gamma, \Delta \vdash \app{M_1}{M_2} : \tau_2} 
\quad
  \prftree
  { \Gamma (x) =  \tau }
  {\Gamma \vdash x:\tau}
\quad
  \prftree
  { b \in \{\ttrue, \ffalse\}}
  {\Gamma  \vdash  b : \linlamBool}
\quad
  \prftree
  {
  \begin{array}{l}
{\Gamma_1   \vdash  M: \linlamBool}\\
{\Gamma _2  \vdash  N: \linlamBool \quad
\Gamma _2  \vdash  N': \linlamBool}
\end{array}
}
  {\Gamma_1,  \Gamma _2 \vdash  \ifSyntax M N N': \linlamBool}
\end{array}
\]

To translate types, we follow the standard tradition of call-by-name
game semantics of interpreting types by "negative
games". Syntactically, we thus interpret a type $ \tau $ by a session
type of the form $\with_{i \in I} T_i$. Such types support an
interpretation of the linear arrow:
\[
  S \linto (\with_{i\in I} T_i) \eqdef \with_{i \in I} (S^\perp  \parallel  T_i)
\]
Types of the $\lambda$-calculus are translated as follows:
$\transl {\linlamBool} \eqdef \start^- \cdot \oplus_{b \in \{\ttrue,
  \ffalse\}} \EmptyType$ and
$\transl{ \tau \linto \tau '} \eqdef \transl \tau \multimap \transl {
  \tau '}$, and typing contexts as:
$\transl{x_1: \tau _1, \ldots, x_n:\tau_n} \eqdef x_1: \transl { \tau _1},
\ldots , x_n: \transl{ \tau _n} $.

For example, the session type associated to linear functions from
booleans to booleans is:
\[
  \transl{\linlamBool \linto \linlamBool} = 
  \transl{\linlamBool} \linto \transl{\linlamBool} =
  \start^- \cdot (\start^- \cdot
  (\ttrue^- \with \ffalse^-) \parallel \ttrue^+ \oplus
  \ffalse^+)
\]

The function awaits for the $\start$ signal from the environment, and
then has a choice: either it returns directly a boolean --- it is a
non-strict function --- or it can ask Context for its argument value
before returning its result.


For terms, the idea is to translate a typing derivation with
conclusion $\Gamma \vdash M : \tau$ into a typing derivation of
$\PIMALL$ whose conclusion is:
$\Typing {\transl{t}^o} \transl{\Gamma}^\perp, o: \transl{\tau}$, where
$o$, the name used to communicate with Context about the return
value, is a parameter of the translation.

However, building directly $\transl t^o$ by induction proved tedious
so we use a slightly stronger inductive invariant. Indeed, the processes
that we will build are all \emph{negative} as well, ie. of the form
$\InputII o {i \in I} {P_i}$ where
$\transl \tau = \with_{i \in i} T_i$. The set $I$ is called the set of
\emph{computation types} of $ \tau $, written $\CompType  \tau $, and we write
$ \tau /i \eqdef T_i$ (for now $I = \{\Start\}$ --- but this property will
not remain true in the extension in \S~\ref{sec:IPA}). It turns out
that constructing $P_i$ is simpler, so from a term
$ \Gamma \vdash M : \tau $, we build a family of processes
$\Typing {\transl { \Gamma \vdash M : \tau }^o_{i}} {\transl
  \Gamma^\perp , o: \tau /i}$ where $i \in \CompType \tau $. Those
processes are put together as follows:
$$\transl{ \Gamma   \vdash  M :  \tau }^o \eqdef \InputII o {i \in \CompType  \tau } {i.\, \transl { \Gamma   \vdash  M :  \tau }^o_i}.$$
The definition of the translation of a linear $\lambda$-terms
(Figure~\ref{fig:translation-affine-calculus}) is now straightforward,
by induction on its structure. From this syntactic translation, we can
derive a semantic interpretation of types and $\lambda $-terms as
games and strategies as follows:
\begin{figure}
  \textbf{Translation of Terms}
{\small
\begin{align*}
  \transl{\abs x M : \tau_1 \linto \tau_2}^o_i
    %
    &\eqdef \Naming o {x, o}.\, \transl M^o_i
  %
  \qquad\quad
  %
  \transl{x:\tau}^o_i
    %
    \eqdef \Output x i.\, 
         \Forwarder x a {\tau/i }
         %
        \quad \qquad
         %
  \transl{b: \linlamBool}^o_{\Start}
    \eqdef
        \Output o b
  %
        \\
    \transl{\app{M_1}{M_2} : \tau_2}^o_i
    %
    &\eqdef \shareInteract x y {}
      {\Split {o} {x, o} {\transl M^o_i}}
      {\transl N^y}
      \\
  %
  \transl{\ifte M N N': \linlamBool}^o_i
    &\eqdef \shareInteract x y {}
      {\transl M^x_\Start}
      {\InputII y {} {\ttrue: \transl N^o_i; \ffalse: \transl {N'}^o_i}}
\end{align*}
}
  \textbf{Macros}
  {\footnotesize
  \[
  \begin{array}{rlll}
    \text{Name} & \text{Definition} & \text{Type} & \text{Given}
    \\
  \Split a {x,y} P & \nu a\, b.\: {(
    P \parallel \Naming b {x', y'}. (\Forwarder x {x'} {} \parallel
    \Forwarder y {y'} {})
  )}
                   & x:T_1, y:T_2
                   & \Typing P {a: T_1 \parallel T_2}
  \\
  \Interact a b P Q &\cut a b \_ {(P \parallel Q)}
                    & \Gamma, \Delta
                    & \Typing P {\Gamma, a:T} \;\;; \Typing Q {\Delta, b:
                    T^\perp}
\end{array}
\]}

%\vspace{-1.5em}
  \caption{Translation from the affine $\lambda$-calculus to $\PIMALL$} 
  \label{fig:translation-affine-calculus}
\end{figure}
%
\[
  \llbracket  \tau  \rrbracket =  \llbracket \transl  \tau  \rrbracket
  \qquad\qquad
  \llbracket M \rrbracket =  \llbracket \transl M^a \rrbracket \quad\text{for some
  $a$.}
\]
\subsubsection*{Correctness of the Encoding} We now show that our
translation characterises $ \beta \eta $-equivalence, defined as the
smallest congruence on typed $ \lambda $-terms containing the well-typed
instances of the rules:
$$\begin{aligned}
 \Gamma   \vdash  ( \lambda x.\, t)\, N &=_{ \beta  \eta } t\subst x N : B &\qquad  \Gamma   \vdash  M &=_{ \beta  \eta } ( \lambda x.\, M\, x) : A  \multimap  B \\
 \Gamma   \vdash  \ifSyntax b {a_{\ttrue}} {a_{\ffalse}} &=_{ \beta  \eta } a_b : \linlamBool &\qquad
 \Gamma   \vdash  M &=_{ \beta  \eta } \ifSyntax M \ttrue \ffalse : \linlamBool
\end{aligned}$$ In the third rule, $b  \in  \{\ttrue, \ffalse\}$ and in
the second $x$ is not free in $t$.

\begin{restatable}[Soundness and Completeness]{theorem}{completenessLambda}
  We have $M =_{ \beta  \eta } N$ if and only if
  $\transl M^a \similarProcesses \transl N^a$ if and only if
  $ \llbracket M \rrbracket  \cong   \llbracket N \rrbracket$.
\end{restatable}
\begin{proof}
  The forward direction is by induction on the rules defining
  $ \beta \eta $. A key property to use is the negativity of
  $\transl M^a$: it always starts by an input on $a$ by construction.
  The converse direction relies on the confluence and normalisation of
  the calculus. Every term $M$ is $ \beta \eta $-equal to its
  $ \eta $-long $ \beta $-normal form. If $M,N$ are in such a normal
  forms, then we prove: $M =_{ \beta \eta } N$ iff
  $\transl M^a \similarProcesses \transl N^a$ iff
  $ \llbracket M \rrbracket \cong \llbracket N \rrbracket$.  See
  Appendix~\ref{app:affinelambda} for details.
\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> minimal.tex <==
\RequirePackage{etex}
\RequirePackage{graphics}
\RequirePackage{array}
\RequirePackage{multirow}
\RequirePackage{xspace} 
\RequirePackage{hyperref} 


%% Encodings
\RequirePackage[T1]{fontenc}
\RequirePackage[utf8]{inputenc}
\RequirePackage{newunicodechar}
\RequirePackage{alltt}
%% AMS
\RequirePackage{amsmath}
\RequirePackage{amsfonts}
\RequirePackage{amsthm}
% \RequirePackage{amssymb} % clashes with acmart on Léo's machine
%% Math in general
\RequirePackage{proof}
\RequirePackage{mathpartir}
\RequirePackage{mathrsfs}
\RequirePackage{stmaryrd}
\RequirePackage{cmll}
\RequirePackage{mathtools}
%% Fancy enumerate list
\RequirePackage{enumerate}
%% TikZ
\RequirePackage{tikz}
\RequirePackage{pgflibraryarrows}
%% XY
\RequirePackage[all]{xy}
%% prftree
\RequirePackage{prftree}


==> nondet.tex <==
This section extends our framework to handle \emph{nondeterminism}. In
\S~\ref{sec:strat_cat}, we introduce a new model that combines \cite{lics15}
and \cite{fossacs18} to have a non-angelic model of nonlinear
computations. In \S~\ref{sec:dill}, we propose our metalanguage for
$\Strat$, denoted as $\PIDiLL$, 
based on Differential Linear Logic ($\DiLL$). In \S~\ref{sec:IPA}, we
give the interpretation of a higher-order language with shared-memory
concurrency.
\subsection{The category $\Strat$}\label{sec:strat_cat}
Traditional models of game semantics tend to have an
\emph{angelic} treatment of nondeterminism: if $M$ is a nondeterministic
program, then $ \llbracket M \rrbracket$ records all the possible maximal executions of
$M$. In particular, it does not record the points where $M$ might get
stuck. Such models equalise $\ttrue + \bot$ and $\ttrue$ (where $+$
represents nondeterministic choice), which shows a loss of
information.
%
In models based on event structures, a similar problem occurs:
moving to nondeterministic $\sim$-strategies does not give an accurate
model of nondeterminism. In \cite{fossacs18}, this problem was
solved by allowing strategies to record internal transitions. Such
internal transitions give rise to \emph{internal events} which can be
used to record \emph{hidden divergences}.

\subsubsection{Essential Strategies}
Formally, such strategies are represented as \emph{partial} maps
$S  \rightharpoonup  A$, and events outside the domain are viewed as internal.

\begin{definition}[\cite{fossacs18}]
An ""essential strategy"" on a game $A$ is a "partial map" $ \sigma  : S  \rightharpoonup  A$ such that:
  \begin{itemize}
  \item if $s  \rightarrowtriangle _S s'$ and $ \sigma \, s,  \sigma \, s'$ are
    incomparable in $A$, then $s$ is non-positive and $s'$ non-negative;
  \item if $x  \in   \config (S)$ and $ \sigma \, x$ can be "extended" by a negative move
    $a  \in  A$, then $x$ can be "extended" by a unique $s  \in  S$ with $ \sigma \, s = a$;
  \item if $s \minconflict s'$, then either both $ \sigma \, s$ and $ \sigma \, s'$
    are defined and negative, or both are undefined;
  \item if $s  \in  S \setminus \dom  \sigma $, then there exists $s'$ such that
    $s \minconflict s'$.
  \end{itemize}
\end{definition}

\noindent
In the first axiom, by non-positive (resp. non-negative) , we mean
that the event is not mapped to a positive event (resp. negative). An
event of $s  \in  S$ is ""internal"" (or invisible) if $ \sigma \, s$ is not
defined, and ""external"" or "visible" otherwise.

The usual "copycat strategy" is an essential strategy (which happens
to be total). Moreover, essential strategies can be composed in a
similar way as strategies.

\begin{theorem}[\cite{fossacs18}]
  There is a category of games and "essential strategies".
\end{theorem}

\subsubsection{Essential $\sim$-Strategies}
To get essential $\sim$-strategies, we simply merge the definitions as
there are very little interactions between the extensions:
\begin{definition}
  Given a "tcg" $\A$, a ""uniformity witness@uwe"" for an "essential strategy"
  $ \sigma  : S  \rightharpoonup  \A$ is an isomorphism family $\tilde S$ such that:
  \begin{enumerate}
  \item $ \sigma $ extends into a map of event structures with symmetry
    $(S, \tilde S)  \rightharpoonup  (A, \tilde A)$;
   \item if $ \theta  : x  \cong  y \in \tilde S$ and $ \sigma \,  \theta $ extends to
    $ \varphi  : x'  \cong  y'$ with $x \subseteq^- x'$, then $ \theta
    $ extends to $ \theta '$ such that $ \sigma \,  \theta ' =
    \varphi $; and 
  \item If $ \theta  : x  \cong  y \in \tilde S$ is the identity on negative
    elements of $x$, then $ \theta $ is the identity on $x$.
  \end{enumerate}
  A ""$\sim$-essential strategy"" on $\A$ is an "essential strategy" $ \sigma $
  on $A$ with a "uniformity witness@uwe" for $ \sigma $.
\end{definition}
As before, uniformity witnesses compose, and most of the structure can
be lifted from $\DetStrat$:
\begin{theorem}
"Thin concurrent games" and "$\sim$-essential strategies" form a
compact-closed category $\intro*{\Strat}$, which has weak (co)products and an
"exponential comonad".
\end{theorem}

\subsubsection{Transitions and weak bisimulation} Event structures
come with a natural notion of transition system, given by
configurations. This can be lifted to the level of strategies. Given
an "essential strategy" $ \sigma : S \rightharpoonup A$, and a
configuration $x \in \config (S)$, we build the "essential strategy"
$ \sigma /x : S/x \rightharpoonup A/ \sigma \, x$ (read $ \sigma $
after $x$) where $S/x$ consists of the events in $S$ which (1) are not
in $x$, but (2) are compatible in $x$, and similarly for
$A/ \sigma \, x$. This construction lifts to "$\sim$-essential
strategies".

We say that $ \sigma : A $ can do a transition to $ \tau $ with
visible actions $y  \in   \config (A)$, written
$ \sigma \mathrel{\intro*{\belowStrategies y}} \tau $, when there exists a
configuration $x \in \config ( \sigma )$ such that
$ \sigma /x \weakIso \tau $ and $ \sigma \, x  \cong  y$ in $\tilde A$. The particular case where
$y = \emptyset$ corresponds to an internal transition and is simply
written $ \sigma  \belowStrategies {}  \tau $.
%
Using this notion of transition, we can define weak bisimulation on strategies:
\begin{definition}
  A \emph{weak bisimulation} is an equivalence relation $\mathcal R$
  between "$\sim$-essential strategies" on the same "tcg" such that if
  $ \sigma \mathcal R \tau $, for all configuration
  $y \in \config ( A )$, if $ \sigma \belowStrategies y \sigma '$,
  then there exists $ \tau '$ such that
  $ \tau \belowStrategies y { \tau '}$ with
  $ \sigma '\mathcal R \tau '$.
   %
We write $\intro*{\Stratwb}$ for the largest weak bisimulation.
\end{definition}
Note that $ \sigma  \weakIso  \tau $ implies $ \sigma \Stratwb  \tau $.
\subsection{A Metalanguage for $\Strat$: $\PIDiLL$}\label{sec:dill}
We present a calculus for $\Strat$ that extends \PILL{} in
\S~\ref{sec:ccll}. For this, we draw inspiration from Differential
Linear Logic which extends Linear Logic with nondeterministic
primitives. $\DiLL$ was introduced to talk about differentiation of
programs, but here we use intuitions coming from $\DiLL$ in terms of
\emph{non-uniform servers}. Earlier, we said that a program of type
$\oc A$ can be seen as a server, able to handle infinitely many
requests. However, the only rule in Linear Logic to build such servers
is the promotion rule, which can represent only \emph{uniform} servers
which handle all requests the same way, without internal state.
$\DiLL$ allows for the possibility of \emph{stateful} servers, and
therefore the possibility of races. This is done by adding two
constructs:
\begin{itemize}
\item \emph{Codereliction} builds a server which will handle
  a unique request. If there are several concurrent requests, one of
  them will be handled and the other ignored (leading to races); and 
\item \emph{Cocontraction} puts two (possibly partial)
  servers together. Requests are then routed to one of the two
  nondeterministically.
\end{itemize}
There is a problem however with this presentation: if we cocontract
two \emph{one-time} servers (obtained by codereliction) and there are
two concurrent requests, then there are several possibilities. The
best case scenario is that each request goes to a different server,
and hence are both handled. The worst case scenario is that they both
go to the same server, and then only one of them will be handled. In
an angelic model, we only see the best case scenario, but in a
non-angelic model we see all cases. To overcome this issue, we add a
single construct, \emph{generalised codereliction}, written
$\Coder a x.\, P$, where $x$ \emph{and} $a$ can be free in $P$:
%
$$P ::= \cdots \mid \Coder a x.\, P \qquad \OpenProc ::= \cdots \mid \Coder a x.\, \OpenProc \qquad \ActionVar^- ::= \cdots \mid \Coder a x.\, X.$$
%
This construct is a mix of codereliction and
cocontraction, which sets up a one-time server on $a$, waits for a
request $x$, and execute $P$. Unlike the usual codereliction, $a$ is
still available in $P$, so that when $P$ has finished handling the
request $x$, $P$ can listen again on $a$. A stateful server can be
written by $\Coder a x.\, P$, and its typing rule is:
\[
\begin{array}{c}
%$P \Coloneqq \dots \mid \Coder a x.\, P$
%\quad and \quad 
\inferrule*[left=ND]
{\Typing P {\Delta , a: \oc A, x: A}}
{\Typing {\Coder a x.\, P} { \Delta , a: \oc A}}
\end{array}
\]
This construct can be used to define the usual nondeterministic sum. 
Given $\Typing {P, Q} { \Delta }$ we define:
$$
\small
\begin{aligned}
P \mathrel{\intro*{\sumProc}} Q \eqdef &\cut a b {\oc (1  \oplus  1)} {
\big(\Coder a x.\, \Input x {\Inl: P; \Inr: Q}
\parallel  (\Der b r.\, \Output r {\Inl} \parallel_{b} \Der b r.\, \Output r {\Inr})\big)}
\end{aligned}$$

\subsubsection*{Interpretation in $\Strat$} To interpret this
extension in $\Strat$, we use a morphism
$c_A : \oc A \parallel A \profto \oc A$.
\begin{wrapfigure}[11]{r}{0.48\linewidth}
  \vspace{-1em}
  \scalebox{0.8} {
  \begin{tikzpicture}
    \matrix[diag, column sep=0] {
      \& \oc A \&  \parallel  \& A \& \rightarrow \& \& \oc A \\[-1mm]
      \& \& \&  \& \& |(bi)| \textbf{box}^-_i \& \& |(bj)| \textbf{box}^-_j \\
       \& \&  \& \& \& |(e1)|  \ast_i  \& \& |(e2)| \ast_j \\
       |(bj')| \textbf{box}^+_{j, i} \& |(bi')| \textbf{box}^+_{i, j} \& \&|(d)| \texttt{a}^-\& \& |(d1)|   \langle \texttt{a},i \rangle ^+\& \& |(d2)|  \langle \texttt{a}, j \rangle ^+ \\
       |(d2')|  \langle \texttt{a},j, i \rangle ^-\& |(d1')|  \langle \texttt{a}, i, j \rangle ^-\\[-1em]
 \& \& \& \& \&       |(d2'')|  \langle \texttt{a},j, i \rangle ^+ \&  \&|(d1'')|  \langle \texttt{a},i, j \rangle ^+\\
    };
    \path (e1) edge[conflict] (e2);
    \path[cause]
    (bi) edge (e1) (bj) edge (e2) (e1) edge (d1) (e2) edge (d2)
    (bi) edge[bend right=20] (bi') (bj) edge[bend right=35] (bj')
    (e1) edge [bend right=20] (bj') (e2) edge[bend right=20] (bi')
    (bi') edge (d1') (bj') edge (d2')
    (d1') edge[bend left=10] (d1'') (d2') edge[bend right=20] (d2'')
    (d) edge (d1) (d) edge[bend right] (d2);
  \end{tikzpicture}
  }
  \vspace{-1em}
  \caption{Strategy $c_A$ for $A = \mathtt{a}^+$}
  \label{fig:cA}
\end{wrapfigure}
The intuition is that requests on the right side race to get forwarded
to $A$; requests that did not win the race are then forwarded to the
left $\oc A$. Since this strategy has a complex operational behaviour,
let us start by an informal description, based on the example where
the game has a single positive move, ie. $A = a^+$. The desired
strategy $c_A$ for a single move game $A = \mathtt{a}^+$ is (partially)
depicted in Figure \ref{fig:cA}.  The strategy starts by waiting for a
request on the rightmost $\oc A$. The different $\mathbf{box}^-_i$ are all
racing together to be considered the \textbf{first} message
acknowledged by $c_A$. Hence, one neutral event per
$\mathbf{box}^-_i$  is triggered when the $i$th message wins the race. If
the $i$th message has won, then the copy of $A$ on the left is put in
contact with the successor of $\mathbf{box}^-_i$, expressed by the
links $a^- \rightarrowtriangle  \langle a, i \rangle ^+$ and
$ \ast _i \rightarrowtriangle  \langle a,i \rangle ^+$. Then, if $i$ has won the race,
it means that any other $j \neq i$ lost. In that case, messages
on the $j$ component are forwarded to the leftmost $\oc A$:
$\mathbf{box}^-_j  \rightarrowtriangle  \mathbf{box}^+_{j, i}$ and
$ \ast _i  \rightarrowtriangle  \mathbf{box}^+_{j, i}$. From there, we have a copycat strategy
between the $i$th copy of $A$ on the left and on the right.
%
Formally, the event structure $C_A$ is defined as:
\begin{description}
\item[Events] are of one of the following form:
\begin{itemize}
\item an event $\mathbf {box}_i^-$ for $i  \in   \mathbb{N} $ mapped to the initial move of the right $\oc A$;
  \item an internal event $ \ast _i$, representing the fact that
    the $i$th request has won the race
  \item an event $\mathbf{box}_{i,j}^{+}$ for $i, j \in \mathbb{N} $,
    corresponding to the forwarding of $\mathbf{box}_i^-$ when $j$ wins the
    race;
  \item an event $ \langle e, i \rangle $ for every $e \in \CC_A$ and $i \in  \mathbb{N} $
    representing the forwarding to $A$ when the race is won by $i$;
  \item an event $ \langle e, i, j \rangle $ for every distinct numbers
    $i, j \neq \mathbb{N} $ and $e  \in  \CC_A$, for forwarding the $i$th
    copy to $\oc A$ when $i$ loses the race to $j$.
  \end{itemize}
\item[Causality] includes the usual causal order on the copies of $\CC_A$, plus the following links:
  \begin{itemize}
  \item $\mathbf{box}^-_i  \rightarrowtriangle   \ast _i$ and $ \ast _i  \leq   \langle e, i \rangle $ for all $e  \in  \CC_A$;
  \item $\mathbf{box}^-_i  \rightarrowtriangle
    \mathbf{box}_{i,j}^{+}$ and 
$\ast _j  \rightarrowtriangle  \mathbf{box}_{i,j}^{+}$ for any
    $i \neq j$: $\mathbf{box}_i^{+, j}$ is played when Opponent made the
    $i$-th request and $j$ won the race; and 
  \item $\mathbf{box}_{i, j}^+  \leq   \langle e, i, j \rangle $ for $e  \in  \CC_A$.
\end{itemize}
\item[Conflict] is generated by asking that the $ \ast _i$ are all in
    mutual conflict.
\end{description}
$C_A$ might not be receptive if $A$ is positive (as in the example),
so that the strategy $c_A$ is obtained by precomposing with copycat to
ensure receptivity. Using this strategy, we let:
$$ \llbracket \Typing{\Coder a x.\, P}{ \Delta , a: \oc A} \rrbracket
= c_A  \odot \left(   \llbracket \Typing P { \Delta , a: \oc A, x: A} \rrbracket :  \llbracket  \Delta  \rrbracket^\perp \profto  \llbracket \oc A \rrbracket  \parallel   \llbracket A \rrbracket \right).$$

\subsubsection*{Preorder} Instead of trying to axiomatise $\weakIso$
in this setting, in presence of nondeterminism, it is more fruitful to
axiomatise the transition relation $\belowStrategies{}$.  We define
the reduction relation $P\intro*{\belowProc} Q$ as the smallest preorder closed
under the rules in Figure~\ref{fig:preorder}. Note that it is not
closed under all prefixes.
%
\begin{figure}
$
\small
\begin{array}{c}
  \infer{\cut a b {T} P \belowProc \cut a b {T} Q}{P \belowProc Q}
  \quad \infer{P' \belowProc Q'}{P' \similarProcesses 
P \belowProc Q \similarProcesses Q'}
\quad 
  \infer
  {\cut a b {\oc T} {\Contr b {b_1} {b_2}.\, P \belowProc \cut a b {\oc T} {\Contr {b} {b_1} {b_2}.\, Q}}}
  {\cut a {b_1} {\oc T} {P} \belowProc \cut a {b_1} {\oc T} {Q}}
\\[2mm]
  \infer{\cut a b {\oc T} {(\Coder a x.\, P \parallel \Der b y.\, Q)
      \belowProc \cut a b {\oc T} {\cut x y {T} {(P \parallel Q)}}}}{}
  \qquad
    \infer{\cut a b {T} {(P \parallel R)} \belowProc \cut a b {T} {(Q \parallel R)}}{\cut a b T P \belowProc \cut a b T Q}
\\[1mm]
\end{array}
$
\caption{Preorder on $\PIDiLL$}
\label{fig:preorder}
\end{figure}
By these rules, we can derive that 
$P + Q  \belowProc  P$ and $P + Q  \belowProc  Q$. 

\begin{restatable}{lemma}{soundnessPreorder}\label{lem:soundnessPreorder}
  For $\Typing {P, Q}  \Delta $, $P \belowProc Q$ implies
  $ \llbracket P \rrbracket \belowStrategies{}  \llbracket Q \rrbracket$.
\end{restatable}
\subsection{Interpretation of a Shared-Memory Concurrent Higher-Order Language} \label{sec:IPA}

\subsubsection*{The Language $\PCFM$} Idealised Parallel Algol
\cite{cia}, $\PCFM$, is an extension of call-by-name PCF with shared
memory concurrency. Types of $\PCF$ are extended by $\UnitType$, the
type of effectful computation, and $\LocType$, the type of
\emph{locations}, ie. references to integers. We use $r, s, \ldots $
to range over variables of type $\LocType$. The terms are extended as follows:
$$M, N ::= \cdots \mid \SkipTerm \mid M; N \mid (M  \parallel  N) \mid \oc M \mid M := N \mid \LetIn r k M$$
with the following standard typing rules:
$$\small 
\begin{aligned}
&\infer{ \Gamma   \vdash  \SkipTerm : \UnitType}{} \qquad \infer{ \Gamma   \vdash  M; N : A}
{ \Gamma   \vdash  M : \UnitType \quad  \Gamma   \vdash  N: A}
\qquad
\infer{ \Gamma   \vdash  M \parallel N : \UnitType}
{ \Gamma   \vdash  M : \UnitType \quad  \Gamma   \vdash  N: \UnitType}
\\&
\infer{ \Gamma   \vdash \oc M :  \mathbb{N} }
{ \Gamma   \vdash  M : \LocType}
\qquad
\infer{ \Gamma   \vdash M := N : \UnitType}
{ \Gamma   \vdash  M : \LocType\quad  \Gamma   \vdash  N :  \mathbb{N} }
\qquad
\infer{ \Gamma   \vdash M := N : \UnitType}
{ \Gamma   \vdash  M : \LocType\quad  \Gamma   \vdash  N :  \mathbb{N} }
\qquad
\infer{ \Gamma   \vdash \LetIn r k M :  \mathbb{N} }
{ \Gamma , r:\LocType  \vdash  M :  \mathbb{N} }
\end{aligned}
$$
In $\LetIn r k M$, $k$ is an integer representing the initial value of
$r$.
\subsubsection*{Operational Semantics} \label{sec:LTS_SC} We recall
the semantics of IPA as given in \cite{cia}. The operational semantics
considers ""programs"", i.e.\ open terms of the form
$r_1: \LocType, \ldots , r_n : \LocType \vdash M : \mathbb{N}$. The
operational semantics has states $\tuple {M, \rho}$ where
$ \Gamma \vdash M : \mathbb{N} $ is a "program" and
$ \mu : \dom{ \Gamma} \rightarrow \mathbb{N}$ is the memory state. It
is given in Figure \ref{fig:LTS_PCFWM}, using the following notion of
evaluation contexts:
$$E[] := [] \mid (P \parallel E) \mid (E \parallel P) \mid []; P \mid \oc E \mid E := n \mid M := E.$$

\begin{figure}
{\small
$
\begin{array}{c}
  \infer{\tuple {(\SkipTerm; M), \rho} \xrightarrow{} \tuple {M, \rho}}{} \quad
\infer{\tuple {M,\rho}  \xrightarrow{ } \tuple {M',  \rho}} {M  \rightarrow_{\text{PCF}} M'}
    \quad 
    \infer{\tuple {\oc r,  \rho } \xrightarrow{} \tuple {k,  \rho }} { \rho (r) = k}
    \quad 
    \infer{\tuple {r:= k,  \rho } \xrightarrow{} \tuple {\SkipTerm,  \rho [r := k]}} {}\\[3mm]
    \infer{\tuple {E[M], \rho} \xrightarrow{ } \tuple {E[M'],  \rho '}} {\tuple {M,  \rho}  \xrightarrow {}  \tuple {M',  \rho '}}
\quad 
    \infer
    {\tuple {\LetIn r k M,  \rho } \xrightarrow{ } \LetIn r { \rho '(r)} {M'},  \rho '}
    {\tuple {M, \rho [r := k]} \xrightarrow{}   \tuple {M', \rho '}}\\[3mm]
  \end{array}
  $}
\vspace{-1.5em}
  \caption{\label{fig:LTS_PCFWM}Operational Semantics for $\PCFM$}
\end{figure}

This operational semantics induces a notion of program equivalence on
closed terms: \emph{weak bisimulation}. Two "programs"
$ \vdash M, N : \mathbb{N} $ are ""weakly bisimilar@wbIPA"" (written
$M \IPAwb N$) when:
\begin{itemize}
\item If $M = n$, then $\tuple {N,\emptyset}  \rightarrow ^* n$
\item If $\tuple {M, \emptyset} \rightarrow \tuple{M',\emptyset}$, then
  $\tuple {N, \emptyset} \rightarrow ^* \tuple{N', \emptyset}$ and
  $M \IPAwb N$.
\end{itemize}



\subsubsection*{Translating $\PCFM$} We first extend the translation of types
    $$\transl {\UnitType} = \start^- \cdot \Done^+ \qquad\qquad
\transl{\LocType} = \start^- \cdot \&\{
    \ReadMsg: \oplus_{n \in \mathbb{N} }\EmptyType, \ 
\WriteMsg(i): \Done^+\}$$

The type $\LocType$ is interpreted as the type of a server waiting for
requests that can be either read requests (answered by a number, the
current value), or write requests, answered by a message acknowledging
the write. The translation of terms is detailed in
Figure~\ref{fig:interpIPA}, and follows closely the intuition of the
interpretation in \cite{cia}. $\LetIn r k M$ is interpreted by
connecting $M$ with a sequential memory server implemented using the
generalised codereliction. The memory server waits for requests and
processes them \emph{in sequence}. If two concurrent requests are
made, then a sequentialisation is picked nondeterministically. (This
behaviour is due to the implementation of $\Coder a x\, P$.)


\newrobustcmd{\MemStrat}{\textsf{mem}}

\newrobustcmd{\ReadFromLoc}[2]{ \Output {#1^{?}} \ReadMsg.\,
  \InputII {#1} {i \in \mathbb{N} } {i.\, #2} }

\newrobustcmd{\WriteToLoc}[3]{ \Output {#1^?}
  \WriteMsg(#2).\, \Wait {#1} {#3} }


\begin{figure}
\textbf{Translation of Terms} \\[-5mm]
\begin{mathpar}\small
  \transl { \Gamma   \vdash  \SkipTerm : \UnitType}^o_i = \Output o \Done
  \and
  \transl { \Gamma   \vdash  \LetIn r k M :  \mathbb{N} }^o_i \eqdef \shareInteract {r} {m} {}
  {\transl M^o_i} {\MemStrat^k_m}
      \and
      \transl { \Gamma   \vdash  M  \parallel  N : \UnitType}^o_\Start \eqdef
      \multicut {x_1\, y_1; x_2\, y_2} {
        \transl M^{x_1}_\Start \parallel_ \Gamma  \transl N^{x_2}_\Start
        \parallel \Wait {y_1} {\Wait {y_2} {\Output o \Done}}
      }
\and
\transl { \Gamma   \vdash  M; N : \UnitType}^o_i \eqdef \shareInteract x y { \Gamma } {\transl M^x_\Start} {\Wait y {\transl N^{o}_i}}
  \and
  \transl { \Gamma   \vdash   \oc M :  \mathbb{N}}^o_\Start \eqdef \transl M^o_{\ReadMsg}
  \and
\transl  {\Gamma   \vdash   M := N : \UnitType}^o_\Start \eqdef
\shareInteract x y { \Gamma }
{\transl N^x_{\Start}}
{\InputII y {n \in  \mathbb{N} } {n.\, \transl M^o_{\WriteMsg(n)}}}
\end{mathpar}

\textbf{Macros}\\[-5mm]
{\footnotesize
\[\begin{array}{rlll}
    \text{Name} & \text{Definition} & \text{Type} & \text{Given} \\
    \MemStrat^k_m & \Coder m x.\, x \with\big\{
  \WriteMsg(i): \Output x \Done.\, \MemStrat^i_m\ ;\ 
  \ReadMsg: \Output x k.\, \MemStrat^k_m
                    \big\} & m: \LocType & k \in \mathbb N\\
    \Wait o P & o \with \Done.\, P &  \Delta , o: \Done^- & \Typing P  \Delta 
  \end{array}
  \]}
%   $$
%   \begin{aligned}
%     \MemStrat^k_m &\eqdef 
% \right\}\Typing{}{m: \LocType} \quad \text{where $k\in \mathbb N$}\\
%   \end{aligned}$$
  \caption{Interpretation of $\PCFWM$ into $\PIDiLL$}
  \label{fig:interpIPA}
\end{figure}


\begin{wrapfigure}[8]{r}{0.43\linewidth}
\vspace{-1.2em}
$
%  \llbracket M \rrbracket =
  \scalebox{0.9}{\begin{tikzpicture}[baseline]
  \matrix[diag] {
    (\UnitType \&  \rightarrow  \& \UnitType) \&  \rightarrow  \& \mathbb B \\[-4mm]
    \& \& \& \& |(q)| \Start^- \\[-5mm]
    \& \& |(q')| \Start^+ \\
    |(q'')| \Start^- \& \& |(d)| \Done^-\\
    |(e1)|  \ast  \& \& |(e2)|  \ast  \\
    |(d'')| \Done^+ \& \& \& \& |(t)| \ttrue^+ \& |(f)| \ffalse^+ \\
  };
  \path [cause]
  (q) edge (q') (q') edge (q'') (q') edge (d)
  (q'') edge (e1) (e1) edge (d'')
  (d) edge (e2)
  (e1) edge (t)
  (d) edge (t)
  (e2) edge (f);
  \path (e1) edge[conflict] (e2);
 \end{tikzpicture}}
 $
\end{wrapfigure}
A first example (without state) of the translation is depicted in
Figure~\ref{fig:overview}, where we write $f[a].\, P$ for
$\Output f \Start.\, \Naming f {a, f}.\, P$ for readability.  Another
more interesting example is the sequential program
$M=\lambda f.\, \text{new $r := 0$ in } f (r := 1); !r = 1$  whose
interpretation is depicted on the right. It tests whether its argument
is a strict function (ie. evaluates its argument before
returning). Its interpretation shows what can happen when $M$ is
evaluated in a concurrent context. In particular, we see that if the
function $f$ provided by the context returns and evaluates its
argument there is a race. This is not possible in $\PCFWM$, but could
be possible in extensions of $\PCFWM$ including control operators.

Our model is adequate with respect to weak bisimulation:
\begin{theorem}[Adequacy]\label{thm:adequacySC}
  For any closed "program" $ \vdash  M:  \mathbb{N} $, we have
  $$M \IPAwb N\qquad\text{if and only if}\qquad  \llbracket M \rrbracket \Stratwb  \llbracket N \rrbracket$$
\end{theorem}

%%% Local Variabls:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

